Constructive Nonlinear Control of Underactuated Systems via Zero Dynamics Policies

Stabilizing underactuated systems is an inherently challenging control task due to fundamental limitations on how the control input affects the unactuated dynamics. Decomposing the system into actuated (output) and unactuated (zero) coordinates provides useful insight as to how input enters the system dynamics. In this work, we leverage the structure of this decomposition to formalize the idea of Zero Dynamics Policies (ZDPs) -- a mapping from the unactuated coordinates to desired actuated coordinates. Specifically, we show that a ZDP exists in a neighborhood of the origin, and prove that combining output stabilization with a ZDP results in stability of the full system state. We detail a constructive method of obtaining ZDPs in a neighborhood of the origin, and propose a learning-based approach which leverages optimal control to obtain ZDPs with much larger regions of attraction. We demonstrate that such a paradigm can be used to stabilize the canonical underactuated system of the cartpole, and showcase an improvement over the nominal performance of LQR.

==> Outputs_and_Normal_Dynamics_v1.tex <==

\begin{comment}
    I think it makes sense to be specific to robotic systems here instead of general control systems. Then we can constructively generate zero dynamics (which I think would be useful for roboticists to see) that are independent of the control input. Also, I think it just gets messy in the general case.

    There exist conditions on the existence of outputs which render the system full-state feedback linearizeable, and therefore do not have zero dynamics \ref{sastry_linearization_1999}. These conditions are difficult to verify, but are in general not satisfied for many control systems of interest.

    For underactuated systems, the rank deficiency of the matrix $\b B$ implies a lack of involutivity of the distribution $\b \Delta(\b x)$, and therefore an inability to choose any output $\b y$ which results in full state feedback linearizeability.
\end{comment}

Consider an $n-$degree of freedom robotic system with coordinates $\b q\in\mathcal{Q}$ and state $\b x = (\b q, \dot{\b q})\in \mathcal{X} \triangleq \mathsf{T}\mathcal{Q}.$ The dynamics can be written in control-affine form as:
\begin{align}
    \dot{\b x} = \underbrace{\begin{bmatrix} \dot {\b q} \\ \b D(\b q)^{-1} \b H(\b q, \dot{\b q}) \end{bmatrix}}_{\b f(\b x)} + \underbrace{\begin{bmatrix} \b 0 \\ \b D(\b q)^{-1} \b B\end{bmatrix}}_{\b g(\b x)}\b u \label{eq:robot_dynamics}
\end{align}
where $\b D : \mathcal{Q} \to \R^{n\times n}$ is the positive-definite mass-inertia matrix, $\b H:\mathcal{X} \to\R^n$ contains the Coriolis and gravity terms, $\b B\in\R^{n\times m}$ is the selection matrix, and $\b u\in\R^m$ is the control input. Many systems of interest -- e.g. legged robots, dexterous manipulators, and systems with strict actuator limits --  are \textit{underactuated}, meaning they have fewer actuators than degrees of freedom ($m < n$). Importantly, restricted actuation authority does not imply a loss of stabilizability; however, achieving stable behaviors requires careful coordination of the actuated degrees of freedom. For the following discussion we assume that $\b B$ has (column) rank $m$, and will be interested in stabilizing these underactuated systems to a goal equilibrium position $\b x^*$.

% (or more generally a control-invariant set $\Omega$),
Towards this goal, it is convenient to construct a collection of outputs $\b y:\mathcal{X}\to \R^p$. The goal will be to construct outputs that, when driven to zero, result in desirable behaviour for the complete system state. In contrast to a common perspective of outputs as observers \cite{kalman_new_1960}, we will instead be interested in outputs for which there exist constructive stabilization techniques. Synthesizing a control input to drive these outputs to zero requires $\b u$ to appear in a derivative of the output in a meaningful way. Consider a time derivative of the output:
\begin{align*}
    \dot {\b y}(\b x) = \underbrace{\frac{\partial \b y}{\partial \b x}\b f(\b x)}_{L_\b f \b y(\b x)} + \underbrace{\frac{\partial \b y}{\partial \b x}\b g(\b x)}_{L_\b g \b y(\b x)} \b u 
\end{align*}
where $L_\b {f}\b y:\mathcal{X} \to \R^p$ and $L_\b {g}\b y:\mathcal{X} \to\R^{p\times m}$ are the \textit{Lie derivatives} of the output $\b y_a$ with respect to the vector fields $\b f$ and $\b g$, respectively. If $L_\b g \b y(\b x) \equiv \b0$, we can attempt to continue differentiating until it is not:
\begin{align*}
    {\b y}^{(\gamma)}(\b x) &= L_\b f^\gamma(\b x) + L_\b gL_\b f^{\gamma-1}(\b x) \b u.
    % \ddot{\b y} &= \underbrace{\b D(\b q)^{-1}\b H(\b q, \dot{\b q})}_{L_\b f^2 \b y_a(\b x)} + \underbrace{\b D(\b q)^{-1}\b B}_{L_\b g L_\b f \b y_a(\b x)}\b u.
\end{align*}
Differentiating the output until the input appears is captured in the following notion of strict relative degree:
\begin{definition}
    \cite{sastry_linearization_1999} \label{def:rel_deg}
    An output $\b y :\mathcal{X} \to \R^p$ for the system \eqref{eq:robot_dynamics} is said to have strict vector relative degree $\gamma\in\mathbb{N}$ at $\b x_0$ if:
    \begin{align*}
        L_{\b g_i}L_{\b f}^k \b y_i(\b x) \equiv 0,\ \ \ \ 0\le k\le \gamma-2
    \end{align*}
    for $i=1,\ldots p$ and the matrix $L_\b g L_\b f^{\gamma-1} \b y(\b x_0)$ is nonsingular.
\end{definition}

Valid relative degree allows the constructive definition of a stabilizing controller, for example the following feedback linearizing controller:
\begin{align}
    \b u = L_\b g L_\b f^{\gamma-1} \b y(\b x)^{-1}(- L_\b f^\gamma \b y(\b x) + \b v), \label{eq:fbl}
\end{align}
whereby the auxiliary input $\b v$ can be chosen such that the resulting output dynamics ${\b y^{(\gamma)}} = \b v$ are exponentially stable. To make this more precise, define the following output coordinates as:
\begin{align*}
    \b \eta(\b x) = \b\Phi_\eta(\b x)= \begin{bmatrix}
        \b \eta^1 \\ \b\eta^2 \\ \vdots \\ \b\eta^{\gamma-1}
    \end{bmatrix} \triangleq \begin{bmatrix}
        \b y(\b x) \\ \dot{\b y}(\b x) \\ \vdots \\ {\b y}^{(\gamma-1)}(\b x)
    \end{bmatrix}.
\end{align*}
where $\b y^{(j)}(\b x) = L_{\b f}^j\b y(\b x)$ for $j=1,\ldots,\gamma-1$ by the relative degree assumption. The output dynamics can be expressed as:
\begin{align*}
	\dot{\b \eta} = \underbrace{\begin{bmatrix}\b 0 & \b I \\ \b 0 & \b 0\end{bmatrix}\b \eta + \begin{bmatrix} \b 0 \\ L_\b f^ \gamma\b y(\b x)\end{bmatrix}}_{\hat {\b f}(\b \eta,\b z)} + \underbrace{\begin{bmatrix} \b 0 \\ L_\b gL_\b f^{\gamma-1}\b y(\b x)\end{bmatrix}}_{\b{\hat g}(\b \eta, \b z)}\b u.
\end{align*}
% Defining the error as $\b e \triangleq \b \eta - \b \eta_d$, 
The output dynamics under the feedback linearizing controller are given by:
\begin{align}
	\dot{\b \eta} = \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 & \b 0 \end{bmatrix}}_{\triangleq \b F}\b \eta+ \underbrace{\begin{bmatrix}\b 0 \\ \b I\end{bmatrix}}_{\triangleq \b G}\b v.
\end{align}
Given positive definite matrices $\b{Q} \in \R^{\gamma\times\gamma}$ and $\b R \in \R^{m\times m}$, we can solve the continuous algebraic Riccati equation (CARE):
\begin{align*}
	\b F^\top \b P + \b P \b F - \b P \b B \b R^{-1} \b B^\top \b P = -\b Q
\end{align*}
for a positive definite symmetric matrix $\b P\in\R^{\gamma\times\gamma}$. This yields an auxiliary input defined by $\b v = -\b R^{-1} \b B^\top \b P \b \eta$ and Lyapunov function $V = \b \eta^\top \b P \b \eta$ certifying the exponential stability of the output coordinates. \red{State somehwere around here that there are a whole class of controllers K which are stabilizing for the system.}




% to exponentially stabilize $\b y_a(\b x)$ to $\b y_d(\b x, t)$. whereby and the.  -- make this point later
% Related to this notion, we now introduce the idea of a desired output being dynamically feasbile:
% \begin{definition}
% 	A desired output $\b y_d:\mathcal{X}\to\R^p$ is \textit{dynamically feasible} if there exists a control input $\b u\in\R^m$ such that:
% 	\begin{align*}
% 		\dot {\b y}_d (\b x) = 
% 	\end{align*}
% \end{definition}

With the goal of stabilizing to an equilibrium point $\b x^* = [\b q^*, \b 0]$, a natural choice of outputs would be $\b y(\b q, \dot{\b q}) = \b q - \b q^*$, whereby we are directly requesting that the joint coordinates converge to a desired state. A quick computation shows that $L_\b {g}\b y(\b x) = \b 0$, and differentiating again, $L_\b {g}L_\b f\b y(\b x) = \b D(\b q)^{-1}\b B$. Because $\b B$ is rank deficient by virtue of the system being underactuated, this output does not have a valid relative degree. 
% , making stabilization of arbitrary goal positions challenging. 
For underactuated robotic systems, it is often challenging if not impossible to find output coordinates which span the complete state space and which can be feedback linearized \cite{bedrossian_nonlinear_nodate}. Even if such coordinates exist, verifying the algebraic conditions required to identify them is difficult \cite{isidori_elementary_1995-1}. In light of this, we will focus on producing coordinates which are of valid relative degree, and which when tracked will result in stability of the complete system.
% A detailed discussion of this can be found in the Appendix. 

Instead of viewing outputs as the primary objectives that we would like to converge to zero, we will use them to characterize the subspace of the system dynamics which the actuators directly effect. With this viewpoint in mind, consider the output zeroing manifold:
\begin{align*}
    \mathcal{Z} = \{ \b x \in \R^n~|~ \b y_a(\b x) = \cdots = \b y_a^{(\gamma-1)}(\b x) = 0\},
\end{align*}
termed the \textit{zero dynamics manifold} \cite{isidori_elementary_1995}. Specifically, we will reason about the vector field which results in invariance of this manifold, defined as:
\begin{definition}
    A manifold $\mathcal{Z}$ is \textit{invariant} if for all $z\in\mathcal{Z}$, we have $\dot {\b x} \in T_\b z \mathcal{Z}$.
\end{definition}
Note that this condition can equivalently be written as:
\begin{align*}
    \langle D\b \eta, \b f(\b x) + \b g(\b x)\b u\rangle = 0
\end{align*}
plugging in the definition of $\dot{\b x}$ and due to the fact that the gradient field of a function whose level set defines a manifold provides a basis for the annihilator of its tangent space.

As the input $\b u^*$ required to keep this manifold invaraint is unique \cite{isidori_elementary_1995}, we will be interested in the case when this $\b u^*$ is also stabilizing on $\mathcal{Z}$. This property will give us composite stability.


\hline

Although producing a coordinate basis for $\mathcal{Z}$ can be challenging in general \cite{isidori_elementary_1995-1}, the structure of $\eqref{eq:robot_dynamics}$ and the outputs defined in \eqref{eqn:outputs} enable us to do this in a straightforward way. Choosing a matrix $\b N\in\R^{(n-m)\times n}$ to be a basis for the left nullspace of $\b B$, coordinates can be generated via:
% which represent a codimension $p$ submanifold in $\R^n$ defining the set of states not directly affected by actuation. 
% . There exist powerful result from geometric nonlinear control gives conditions on the existence of such coordinates, but these often result in verifying messy algebraic equalities. 
% Conveniently, for robotic systems with the structure of $\eqref{eq:robot_dynamics}$ such coordinates can be constructively generated
% by choosing the matrix $\b N\in\R^{(n-m)\times m}$ to be a basis for the left nullspace of $\b B$. With this, coordinates are given by:
\begin{align*}
    \b z(\b x) = \b\Phi_\b z(\b x) \triangleq\begin{bmatrix} \b N \b q \\ \b N \b D(\b q) \dot{\b q}\end{bmatrix}.
\end{align*}
These coordinates were chosen such that $\frac{d\b\Phi_\b z}{d \b x} \b g(\b x) \equiv \b 0$; as such, this mapping explicitly decomposes the state space into a subspace that can directly be controlled, and one that cannot. To transfer conclusions from the $(\b \eta, \b z)$ space to the original state space, we require that the map between them is bijective, as summarized in the following statement:
\begin{proposition}
\label{prop:bijection}
The mapping $\b \Phi$ defined as:
\begin{align*}
    \begin{bmatrix} \b \eta(\b x) \\ \b z(\b x)\end{bmatrix} = \b \Phi(\b x) \triangleq \begin{bmatrix} \b \Phi_\eta(\b x) \\ \b\Phi_z(\b x)\end{bmatrix},
\end{align*}
is a diffeomorphism between $\mathcal{X}$ and $\mathcal{N}\times\mathcal{Z}$.
\end{proposition}

% Finally, applying the feedback linearizing controller from \eqref{eq:fbl}, 
Finally, the associated dynamics in $(\b \eta, \b z)$ space are:
\begin{align}
    % \dot{\b \eta} &= \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 &\b 0 \end{bmatrix} \b \eta + \begin{bmatrix}\b 0 \\ L_{\b f}^\gamma\b y_a(\b \Phi^{-1}(\b \eta, \b z)) \end{bmatrix}}_{\hat{\b f}(\b \eta, \b z)} + \underbrace{\begin{bmatrix}\b 0 \\ L_\b gL_{\b f}^\gamma-1\b y_a(\b \Phi^{-1}(\b \eta, \b z))\end{bmatrix}}_{\hat{\b g}(\b \eta, \b z)}\b u, \\
    % \dot{\b \eta} &= \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 &\b 0 \end{bmatrix}}_{\triangleq\b F} \b \eta + \underbrace{\begin{bmatrix} \b 0 \\ \b I \end{bmatrix}}_{\triangleq\b G} \b v, \ \ \ \ \ \ 
    % \dot{\b z} = \underbrace{D\Phi_z \b f(\b \Phi^{-1}(\b \eta, \b z))}_{\triangleq\b \omega(\b \eta, \b z)}.
    \dot{\b \eta} &= \hat{\b f}(\b \eta, \b z) +\hat{\b g}(\b \eta, \b z) \b u, \ \ \ \ \ \ 
    \dot{\b z} = \underbrace{D\Phi_z \b f(\b \Phi^{-1}(\b \eta, \b z))}_{\triangleq\b \omega(\b \eta, \b z)}. \label{eqn:zd}
\end{align}
Conveniently, for the proposed choice of outputs and normal coordinates, constructing the function $\b\Phi^{-1}$ is straightforward.
The next section will discuss the benefit of decomposing the system this way as a method of structuring stabilizing feedback policies.

With this viewpoint in mind, consider the following outputs:
\begin{align}
    \b y_a(\b q) = \b B^\top \b q, \label{eqn:outputs}
\end{align}
whereby $L_\b g L_\b f \b y_a(\b x) = \b B^\top \b D(\b q)^{-1} \b B$ is an $m\times m$ block on the diagonal of a positive definite matrix, and is therefore full rank. Thus, these outputs have strict vector relative degree 2, and can be constructively stabilized via collocated feedback linearization. As we care about stabilizing $\b x$ and not just $\b y_a(\b x)$, however, we would like to know how stabilizing the outputs affects the complete system state.

==> ZD_sec_A_old.tex <==
Much of control theory is concerned with the stabilization of outputs. Even for nonlinear systems, there exist many well founded theoretical tools to stabilize the outputs of a system. For underactuated systems, once outputs have been stabilized, there exist residual dynamics. There are several works in control theory which aim to demonstrate that these residual dynamics, often termed zero dynamics (as the dynamics which remain in the system when the outputs are zero) have some properties, for instance boundedness. In many cases, results rely on the assumption that these residual dynamics are stable, or at best optimize local stability criteria on the residual dynamics (HZD). We propose an alternate paradigm, where the primary focus is identification of a surface whose zeroing dynamics are stable. We parameterize the surface in a way such that once identified, output tracking tools can be used to stabilize the surface, giving composite stability of the overall system by construction. 

With the goal of stabilizing the full system state in the light of the previous discussion, we introduced the concept of a Zero Dynamics Policy: a function $\func:\mathcal{Z}\to\mathcal{N}$ mapping between the underactuated and actuated coordinates, for which stabilizing $\b \eta \rightarrow \b \psi(\b z)$ (which can be done constructively) results in stability of the overall system. This approach draws inspiration from many successful results in robotics \red{raibert, centroidal MPC, backstepping, sliding mode control}. We first define and lay out desired properties of the \emph{zeroing manifold}induced by the function $\psi$. Next, under the zeroing manifold, we prove that for controllable systems of the form \ref{eq:robot_dynamics}, such functions are guaranteed to exist locally around the origin. Finally, we introduce an algorithmic, learning-based approach leveraging optimal control to synthesize zero dynamics policies. 

Let the output be defined as $\b y = \b \eta^1$

Consider a nonlinear system \ref{eq:general_dyn}, with a vector relative degree $\gamma$ output, placed into normal form \ref{eqn:zd}. As discussed previously, we look for a mapping $\psi: \mathcal{Z} \rightarrow \mathcal{N}$ with desirable properties: consider the manifold
\begin{align*}
    \mathcal{M} \triangleq \{(\b \eta, \b z)\in \mathcal{N}\times\mathcal{Z}~|~ \underbrace{\b \eta - \func(\b z)}_{\triangleq h(\b \eta, \b z)}= \b 0\}
\end{align*}
which is an embedded submanifold of $\mathcal{N} \times \mathcal{Z}$, of codimension $\dim{\mathcal{Z}}$. Our control approach will be to design $\mathcal{M}$ in such a way that stabilizing $\mathcal{M}$ results in stabilization of the entire system. To accomplish this, we require a few additional properties of $\mathcal{M}$: the first is that the it can be rendered invariant through control action.
\begin{definition}
    A manifold $\mathcal{M}$ is said to be controlled invariant under a given smooth controller $\b u(\b \eta, \b z)$ if the dynamics under $\b u$ are tangent to the manifold, $\b F(\b \eta, \b z) + \b G(\b \eta, \b z) \b u(\b \eta, \b z) \in T_{\b \eta, \b z}\mathcal{M}$. 
\end{definition}

A necessary and sufficient condition for invariance of the manifold under a controller $\b u(\b \eta, \b z)$ is
\begin{equation*}
    \left\langle Dh(\b\eta, \b z), \b F(\b \eta, \b z) + \b G(\b \eta, \b z) \b u(\b \eta, \b z)\right\rangle = 0
\end{equation*}
\begin{equation*}
    \left\langle \begin{bmatrix}
        I & -\frac{d \b \psi}{d\b z}
    \end{bmatrix}^\top, \begin{bmatrix}
        \b \hat{f}(\b \eta, \b z) + \b \hat{g}(\b \eta, \b z) \b u(\b \eta, \b z) \\
        \omega(\b\eta, \b z)
    \end{bmatrix}\right\rangle = 0
\end{equation*}
since the gradient field of a function whose level set defines a manifold provides a basis for the annihilator of its tangent space.

Next, we require that the dynamics of the system restricted to the manifold are stable. 
\begin{lemma}
    The restriction of the dynamics to the manifold are unique, regardless of the controller used to render the manifold invariant.
\end{lemma}
\begin{proof}
    On the manifold, we have $\b \eta = \b \psi(\b z)$. The $\b z$ dynamics are therefore 
    \begin{equation} \label{eqn:zd_surf_dynamics}
        \dot{\b z} = \b\omega(\b\psi(\b z), \b z)
    \end{equation}
    These dynamics are autonomous (do not depend on $\b u$), and $\b z$ completely parameterizes the manifold. Since $\b \omega$ is locally Lipshitz continuous by assumption, solutions are unique and the manifold has unique dynamics. 
\end{proof}
\begin{definition}
    A manifold $\mathcal{M}$ which can be rendered invariant is stable if the dynamics restricted to the manifold \eqref{eqn:zd_surf_dynamics} are stable.
\end{definition}

The final condition that we require of $\mathcal{M}$ is that it is able to be constructively rendered attractive. This notion is captured by the idea of valid relative degree, posed in Definition \ref{def:rel_deg}.
\begin{lemma}
    Assume the manifold $\mathcal{M}$ is controlled invariant. Consider the signal $e_1 = \b \eta_1 - \b \psi_1(\b z)$. If $\b e_1 \equiv 0$, then $(\b \eta, \b z) \in \mathcal{M}$. Furthermore, if $\b e_1$ or any of its first $\gamma - 1$ derivatives are non-zero, then $(\b\eta, \b z) \notin \mathcal{M}$
\end{lemma}
\begin{proof}
    Consider a point on the manifold. Since the $\b\eta$ coordinates are simply a chain of integrators, and using the fact that $\eta_i = \psi_i(z)$, when on the manifold we have
    \begin{equation} \label{eqn:psi_integrator_chain}
        \psi_{i+1}(z) = \eta_{i+1} = \dot{\eta_i} = \frac{d}{dt}\psi_i(z)
    \end{equation}
    via induction, this implies that $\psi$ also satisfies an integrator structure \emph{on the manifold} (note that this is not true off the manifold, as the leftmost equality does not hold). 
    
    Consider the value of $e_1$ and its derivatives on the manifold. Trivially, $e_1=0$ since $\eta_1 = \psi_i(z)$. Computing the first derivative
    \begin{align*}
        \dot{e_1} = e_2 &= \dot{\eta_1} - \frac{d}{dt} \psi_1(z) \\
        &= \eta_2 - \psi_2(z)\\
        &= 0
    \end{align*}
    Applying \eqref{eqn:psi_integrator_chain} inductively demonstrates that $e_1$ and all of its derivatives are zero on $\mathcal{M}$. 

    Now, consider a point off the manifold. There must exist at least one index $i$ for which $\eta_i \neq \psi_i(z)$.
    
\end{proof}
\begin{definition}
    The manifold $\mathcal{M}$ can be constructively be rendered attractive if the signal $\b e_1: \b\eta_1 - \b\psi_1(\b z)$ has valid relative degree (Definition \ref{def:rel_deg}).
\end{definition}

The valid relative degree of $\b e_1$ implies that $\b e_1$ can be driven to zero constructively, using, for instance, a feedback linearizing controller; this renders the manifold attractive. We will define $\mathcal{K}$ to be the set of controllers which exponentially stabilize $\b e_1$ to zero, driving the system to the manifold $\mathcal{M}$.
\begin{lemma} \label{lem:eta_from_e}
    Assume the output $y = \eta_1 - \psi_1(z)$ has valid relative degree, and $\b e = \begin{bmatrix}
        y & \hdots & y^{\gamma - 1}
    \end{bmatrix}^\top$. Then there exists a mapping $\Gamma: \mathcal{E} \times \mathcal{Z} \rightarrow \mathcal{N}$, which takes $(\b e, \b z) \mapsto \b\eta$.
\end{lemma}
\begin{proof}
    Consider relative degree two. Trivially, $\eta_1 = e_1 + \psi_1(z)$. It remains to show that $\eta_2 = \Gamma_2(e, z)$. Consider the definition of $e_2$:
    \begin{align*}
        e_2 &= \dot{e_1} \\
        &= \eta_2 - \frac{d\psi_1}{dz} \omega(\eta, z)
    \end{align*}
    We can verify the existence of $\Gamma_2$ via the implicit function theorem. Taking
    \begin{equation*}
        0 = \eta_2 - \frac{d\psi_1}{dz} \omega\left(\begin{bmatrix}
            e_1 + \psi_1(z) \\ \eta_2
        \end{bmatrix}, z\right) - e_2 = \Lambda(\eta_2, e, z)
    \end{equation*}
    The implicit function theorem guarantees the existence of $\eta_2 = \Gamma_2(e, z)$ as long as
    \begin{equation*}
        \frac{d\Lambda}{d\eta_2} = 1 - \frac{d\psi_1}{dz} \frac{d\omega}{\eta_2}
    \end{equation*}
    is nonzero. However, this is the same as the condition for valid relative degree of the output; therefore, by assumption of valid relative degree, $\Gamma$ exists and the mapping is well defined. 
\end{proof}
\begin{theorem} \label{thm:composite_lyap}
    If there exists a suitable $\b \psi$ such that $\mathcal{M}$ satisfies (1)  controlled invariant, (2) dynamics restricted to the surface are stable, and (3) can be rendered attractive, then the system is stable under any controller $\b u \in \mathcal{K}$.
\end{theorem}
\begin{proof}
    Apply any controller in $\mathcal{K}$ to the system. This controller exponentially converges $e = \begin{bmatrix}
        e_1 & \hdots e_{\gamma - 1}
    \end{bmatrix}^\top \rightarrow 0$. By converse Lyapunov, we have the existence of a Lyapunov function $V_e(e)$, certifying the stability of $e$:
    \begin{align*}
        k_1 \|e\|^2 \leq V_e(e) &\leq k_2 \|e\|^2 \\
        \dot{V}_e(e) &\leq -k_3 \|e\|^2 \\
        \left\| \frac{dV_e}{de} \right\| &\leq k_4 \|e\|
    \end{align*}
    Additionally, the controller renders $\mathcal{M}$ forward invariant. Any point on $\mathcal{M}$ has $e=0$, so an exponentially convergent controller will maintain $e\equiv 0$. Therefore, under the same controller, the system restricted to the surface will be exponentially stable, by assumption (2). By converse Lyapunov, there exists a Lyapunov function $V_z(z)$ certifying stability of the $z$ dynamics on $\mathcal{M}$:
    \begin{align*}
        k_5 \|z\|^2 \leq V_z(z) &\leq k_2 \|z\|^2 \\
        \dot{V}_z(z) &\leq -k_3 \|z\|^2 \\
        \left\| \frac{dV_z}{dz} \right\| &\leq k_4 \|z\|
    \end{align*}
    Consider the candidate composite Lyapunov function $V(\eta, z) = \sigma V_e(e) + V_z(z)$. This function satisfies 
    \begin{equation*}
        \min\{\sigma k_1, k_5\} \|e, z\|^2 \leq V(e, z) \leq \max\{\sigma k_2, k_6\}
    \end{equation*}
    Additionally, use Lemma \ref{lem:eta_from_e} to rewrite the $z$ dynamics in terms of $e$ and $z$:
    \begin{equation*}
        \dot{z} = \omega(\eta, z) = \omega(\Gamma(e, z), z) = \Tilde{\omega}(e, z)
    \end{equation*}
    Computing the time derivative of $V$:
    \begin{align*}
        \dot{V}(e, z) &= \sigma\frac{dV_e}{de} \dot{e} + \frac{dV_z}{dz} \Tilde{\omega}(e, z) \\
        &= \sigma \frac{dV_e}{de} \dot{e} + \frac{dV_z}{dz}\Tilde{\omega}(0, z) + \frac{dV}{dz}\left(\Tilde{\omega}(e, z) - \Tilde{\omega}(0, z) \right) \\
        &\leq -\sigma k_3 \|e\|^2 - k_7 \|z\|^2 + k_8 L_\omega \|e\| \|z\| \\
        &= -\begin{bmatrix}
            \|e\| \\ \|z\|
        \end{bmatrix}^\top \begin{bmatrix}
            \sigma k_3 & -\frac{k_8 L_\omega}{2} \\
            -\frac{k_8 L_\omega}{2} & k_7
        \end{bmatrix}\begin{bmatrix}
            \|e\| \\ \|z\|
        \end{bmatrix}
    \end{align*}
    Choosing $\sigma > \frac{k_4^2 L_\omega^2}{2k_3 k_7}$ renders the matrix positive definite, and certifies $\dot{V}(e, z) \leq -\lambda_{min} \|e, z\|^2$. The stability of the composite system is certified. 
\end{proof}

==> arXiv/Sections/Conclusion.tex <==
\vspace{-3mm}\section{Conclusion}

In this work, barrier functions, machine learning, and dimension reduction via zero dynamics were combined to provide a novel way of generating walking behaviors for a bipedal robot. 
Our approach used learning in two places: policy design and residual dynamics modeling via data collection on hardware.  
The proposed method culminated in a demonstration of agile and robust locomotion on hardware. Future work includes studying more complex robots, online learning, as well as policy learning for new behaviors (e.g., walking up stairs). 







==> arXiv/Sections/Introduction_v2.tex <==


Realizing bipedal locomotion on legged robots is difficult due to the compounded complexity of nonlinear underactuated dynamics coupled with the hybrid nature of walking. 
Underactuation makes the application of classic nonlinear control approaches challenging, necessitating the use of offline optimization to generate periodic walking gaits. Due to the combinatorics of contact conditions resulting from the hybrid dynamics, feasibility of this optimization problem requires either fixing the contact times and positions (which can be vulnerable to perturbations) or expensive planning through the set of possible contact points.
Pushing this offline optimization problem online allows for reactive controllers but requires the use of reduced-order models that limit formal guarantees. 
Despite impressive examples of implementations that deal with bipedal walking in practice, general bipedal locomotion with formal performance guarantees remains an open problem.

\textbf{Prior Work in Control.} In the control literature, bipedal locomotion follows two general branches: walking with guarantees of stability and predictive control approaches. 
Walking with guarantees usually relies on solving optimization programs offline to generate stable (periodic) gaits \citep{Hereid2017FROST}.
Above all, this approach relies on constraining walking to be a periodic orbit with assumed exponential stability on the underactuated coordinates of the robot.
This underlying assumption can be problematic in safety critical settings when the gait must satisfy hard constraints such as staying on predetermined stepping stones \citep{csomay-shanklin_episodic_nodate,NGUYEN2015147} and also precludes different walking modes such as period-two walking and, more generally, aperiodic locomotion \citep{xiong2019orbit,ames_first_2017}.
This is particularly important given that disturbance rejection can require aperiodic behaviors \citep{4307016}.
Predictive control approaches on the other hand are able to avoid the aforementioned limitations by planning trajectories and/or policies online, and have shown great promise for quadrupedal robots \citep{di2018dynamic, grandia2019feedback}. Their application to bipedal robots is comparatively sparse however, and has predominantly required static stability \citep{tedrake2015closed,scianca2020mpc} or simplified models to mitigate the computational complexity \citep{kuindersma2016optimization, apgar2018fast, xiong20213d}. This leads to challenges when seeking formal guarantees for dynamic bipedal locomotion in the presence of model mismatch between the planning and low-level control layers.

\textbf{Prior Work in Learning.}
Prior work in machine learning has produced impressive results towards realizing legged locomotion using reinforcement learning \citep{lee_learning_2020,DBLP:journals/corr/abs-2011-01387,DBLP:journals/corr/abs-2103-15309,heess2017emergence}.
These methods use relatively simple reward functions along with sophisticated simulations to generate large amounts of data to train a policy capable of traversing a variety of terrains.
Still, these algorithms can be fragile when facing environments outside of the training dataset and are data inefficient due to not exploiting the full dynamics structure.
These challenges make it difficult to reliably apply these methods on complex hardware systems.
Other works have attempted to use reinforcement learning to train a parameterization of a Control Barrier Function (CBF) Control Lyapunov Function (CLF) Quadratic Program Controller (CBF CLF QP) \citep{choireinforcement,csomay-shanklin_episodic_nodate}. Differing from these works, this paper does not learn a projection of the modeling error onto the CLF and CBF constraints; instead we learn the projection of our modeling error on the zero dynamics. Furthermore, we do not specify a desired trajectory but rather provide a set of barriers that imply walking as emergent behavior.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/OverviewFigure_v5.pdf}
    \vspace{-20pt}
    \caption{A depiction of the Neural Gaits framework. \textbf{Left:} Designing barrier function candidates that we use to formally describe walking. \textbf{Middle:} Training a policy capable of satisfying all the barrier condition in the zero dynamics state space where the constraint is enforced.
    \textbf{Right:} Collecting hardware data to train a residual zero dynamics model. We then refine the policy episodically using the augmented model.}
    \label{fig:overview}
\end{figure}

\textbf{Our Contributions.}
In this work we are instead interested in automatically discovering good walking policies by integrating learning with control-theoretic formulations of stable walking.
Rather than optimizing a simple reward/cost function, our policies learn to satisfy algebraic forward set invariance conditions, certified by control barrier functions, that characterize good walking behavior (as illustrated in the first block of \cref{fig:overview}).
This integrated approach offers three potential benefits.
First, we are able to certifiably handle impact uncertainty by training policies that satisfy conditions for good impact behavior on a region surrounding the nominal impact guard.
Second, our sampling-based approach is focused on a lower-dimensional state space which can be more data efficient and, under the assumption that walking is a form of set invariance, can produce policies with performance certificates.
The latter point contrasts with offline or predictive trajectory generation perspectives where, even if you enforce control theoretic conditions over the predicted trajectory, you cannot certify performance over a set surrounding the trajectory, thereby breaking set invariance guarantees even under small perturbations. Furthermore, leveraging zero dynamics significantly reduces the dimensionality of the learning problem while remaining compatible with the use of control barrier functions, thus enabling guarantees for the full-order system (see \cref{sec:learn_eps}). 
Third, rather than relying on the artificial constraint of periodic orbits, we are able to characterize walking solely as set invariance while retaining stability guarantees. 
The combined benefit is a reliable and efficient approach for designing gaits that can be deployed on hardware platforms.

Our proposed approach, called \emph{Neural Gaits}, is composed of two learning modules.
The first module trains a policy (which generates walking gaits) to minimize the violations of forward set invariance, implemented using control-theoretic barrier conditions as shown in the second block of \cref{fig:overview}.
In doing so, we can guarantee forward set invariance, which implies (under suitable assumptions) indefinite stable walking.
The second module trains a residual dynamics model to refine imperfections of the current dynamics model based on hardware experiments as represented by the arrow between block three and two in \cref{fig:overview}.
Both modules are then iterated on episodically with hardware experiments in the loop.
We also build upon recent work in training ODE-based systems (of which locomotive walking is an instance of), such as LyaNet \citep{lyanet} and Neural ODEs \citep{chen_neural_2019}, in order to develop an effective training approach.


We empirically demonstrate our approach on the AMBER-3M hardware platform \citep{ambrose_toward_2017} with partially unknown dynamics. We show that the resulting policy is capable of making the robot walk under significant model mismatch and adapts to improve barrier satisfaction across episodes. To the best of our knowledge, this is the first successful demonstration of integrated learning and control for bipedal locomotion with stability guarantees.






















==> arXiv/Sections/Preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
We provide a brief introduction of zero dynamics, hybrid dynamical systems, and control barrier functions, which are necessary fundamentals to understand the proposed formulation in \cref{sec:proposed_method}.
\subsection{Output and Zero Dynamics}
\label{sec:prelim:output_and_zdyn}
Consider the general nonlinear ordinary differential equation:
\begin{align}
    \dot{\gs} &= \gf(\gs, \gu),\quad\quad
    \gs(0) = \gs_0, \label{eq:general_dyn}
\end{align}
with states $\gs \in \gX \subseteq \R^n$, inputs $\gu \in \gU \subseteq \R^m$, and dynamics $\bm f: \gX \times \gU \to \R^n$ with $\bm f$ locally Lipschitz in both arguments. For mechanical systems, we specialize to the control-affine case:
\begin{align}
    \label{eqn:eom}
    \dot{\bm x}  &= \bm f(\bm x) + \bm g(\bm x) \bm u,
\end{align}
where $\bm f: \pX \to \R^n$ and $\bm g: \pX \to \mathbb{R}^{n\times m}$ are assumed to be locally Lipschitz. Denoting a parameter in a parameter space $\bm \theta\in\bm\Theta$, we can define a collection of $k$ outputs $\bm y: \pX \times \bm{\Theta} \to \R^k$ parameterized by $\bm \theta$ that we would like to converge to zero as:
\begin{align}
\label{eq:output_coords}
        \bm y(\bm x; \bm \theta) &= \bm {y_a}(\bm x) - \bm {y_d}(\bm x; \bm{\theta}),
\end{align}
where $\bm{y_a}:\pX\to\R^k$ are the measured outputs, and $\bm{y_d}:\pX \times \bm{\Theta} \to\R^k$ are the desired outputs. For locomotion, the outputs are typically taken either as joint angles (as done in this work), or as center of mass and foot positions. For the policy $\bm y_d$ learned in this work and shown in the center block of \cref{fig:overview}, $\bm{\theta}$  corresponds to neural network parameters.
Although all the concepts may be extended to systems with valid decomposition into output and zero dynamics coordinates (which includes all mechanical systems), for simplicity the remainder of the exposition will be restricted to the setting used in this work, namely with $k=4$ and $\bm y_a$ taken to be the actuated joint angles of the robot. For a complete description of output coordinates and zero dynamics, we  refer to \citep{isidori_elementary_1995}.

Given these outputs $\bm y$, we can separate the actuated and the unactuated coordinates for the robot, which are shown in Figure~\ref{fig:hzd_decomposition}a. As these outputs are \textit{vector relative degree} 2, we can define error coordinates $\bm \eta_i:\pX \to \mathcal{N}_i \subseteq \R^2$ for $i=1,\ldots 4$ as $\bm \eta_i = \begin{bmatrix} y_i^\top, & \dot{y}_i^\top \end{bmatrix}^\top$, as well as the collection of errors $\bm \eta = \begin{bmatrix} \bm\eta_1^\top, & \dots, & \bm\eta_4^\top \end{bmatrix}^\top$. Then, there exist 2 linearly independent functions $z_i:\pX\to\mathcal{Z}_i\subseteq\R$ for $i=1,2$ such that $\nabla_{\mathbf{x}}z_i(\bm x)g(\bm x) \equiv 0$, and  $\nabla_{\bm x} z_i(\bm x)$ is linearly independent from $\nabla_{\bm x} \eta_{i,j}(\bm x)$ for $i=1,\ldots,4$ and $j=1,2$.%
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/Fig2_v2.pdf}
    \vspace{-20pt}
    \caption{
    \textbf{a)} The continuous and discrete phases of the robot, with actuated ($\bm \eta$) and unactuated ($\bm z$) coordinates depicted. 
    \textbf{b)} The diffeomorphism $\bm \Phi$, and the relationship between state space coordinates and output/zero dynamics coordinates.
    }
    \label{fig:hzd_decomposition}
\end{figure}
We can then construct a diffeomorphism\footnote{. This is differentiable in the first argument and differentiable almost everywhere in the second argument.} $\bm \Phi:\pX\times\boldsymbol\Theta\to\mathcal{N}\times \mathcal{Z}$:
\begin{align*}
\begin{bmatrix}\bm \eta \\ \bm z\end{bmatrix} = \begin{bmatrix}\bm \Phi_{\bm \eta}(\bm x; \bm \theta) \\ \bm \Phi_{\bm z}(\bm x)\end{bmatrix} \triangleq \bm \Phi(\bm x; \boldsymbol \theta),~~\qquad\bm x = \bm \Phi^{-1}\left(\begin{bmatrix}\bm \eta\\ \bm z\end{bmatrix}; \boldsymbol \theta\right),
\end{align*}
as shown in Figure~\ref{fig:hzd_decomposition}b. Under this coordinate transformation, the system dynamics become:
\begin{align}
\label{eq:diff_dyn_projection}
    \begin{bmatrix}
    \dot{\bm \eta} \\ \dot{\bm z}
    \end{bmatrix} = 
    \begin{bmatrix}
    \bm{\hat{f}}(\bm \eta; \bm \theta) + \bm{\hat{g}}(\bm \eta; \bm \theta)\bm u \\
    \bm{\omega}(\bm \eta, \bm z; \bm \theta)
    \end{bmatrix},
\end{align}
where $\bm{\hat{f}}, \bm{\hat{g}}$ and $\bm{\omega}$ are the projection of the dynamics through the diffeomorphism $\bm \Phi$.%



The \textit{zero dynamics manifold} $\mathcal{Z}\subset\pX$ is thus the space where errors have been driven to zero:
\begin{align*}
\mathcal{Z} = \{\bm x\in \gX:~\bm \eta (\bm x) = 0\},
\end{align*}
as seen in Figure~\ref{fig:hzd_decomposition}a. Observe that for $\bm z\in\mathcal{Z}$, we have that $\dot{\bm z} = \bm{\omega}(\bm 0, \bm z;\bm \theta)$. The power of the method of zero dynamics lies in that it allows for guarantees about the full nonlinear dynamics by considering only a subspace of significantly smaller dimensionality \citep{isidori_elementary_1995}. Notice that although the input does not appear in the zero dynamics $\bm \omega$ in \eqref{eq:diff_dyn_projection}, the parameters of the policy $\bm \theta$ do. This realization motivates the use of the policy as a way to influence the zero dynamics and enforce the desired barrier functions, as introduced below. Finally, in this work we will learn residual dynamics $\varepsilon(\bm z)$ on the zero dynamics manifold for a corrected zero dynamics $\dot{\bm z} = \bm{\omega}(\bm 0, \bm z) + \varepsilon(\bm z)$ that compensate for modeling error. This process is captured in the episodic iteration of \cref{fig:overview}. 


\subsection{Hybrid Dynamics}
Walking consists of continuous evolution with discrete impacts occurring as contact is made and broken (e.g, the feet with the ground). This sequence of continuous and discrete dynamics is shown in Figure~\ref{fig:ZDandBarriers}a can be modeled in the language of \textit{hybrid systems} as:
\begin{align*}
    \hybrid = \begin{cases}\dot{\bm x} = \bm f(\bm x) + \bm g(\bm x) \bm u & \bm x\in \mathcal{D}\backslash\mathcal{S} \\ \bm x^+ = \Delta(\bm x^-) & \bm x\in\mathcal{S}\subset\mathcal{D},\end{cases}
\end{align*}
where $\mathcal{D} \subset\mathcal{X}$ is the domain where $\gs(t)$ evolves. The \textit{guard}, $\mathcal{S}\subset\mathcal{X}$, corresponds to the set of states where the foot comes in contact with the floor. The \textit{reset map}, $\Delta:\mathcal{S} \to \mathcal{D}$ models the instantaneous sign flip of velocities observed when two rigid bodies collide (the foot with the ground). 
Furthermore, $\hybrid$ can be projected through the diffeomorphism $\bm \Phi$ to exploit the  decomposition into output and zero dynamics. For more details, we refer to \citep{westervelt_feedback_2018}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{Figures/Fig3_v2.pdf}
    \vspace{-20pt}
    \caption{\textbf{a)} The guard $\mathcal{S}$, reset map $\Delta(\mathcal{S})$, and safe set $\mathcal{C}_\mathcal{Z}$ are visualized in the state space decomposed into output $\mathcal{N}$ and zero dynamics $\mathcal{Z}$ coordinates. \textbf{b)} A safe set defined as regions of the state space (gray square) where $h$ is positive (blue region). Satisfying the CBF condition implies that the flows/discrete updates of the system will not leave the safe set (although may approach the boundary). Violations imply a flow that could potentially leave the safe set.}
    \label{fig:ZDandBarriers}
\end{figure}

\subsection{Control Barrier Function Certificates}
\label{sec:cbf}
Barrier function certificates allow us to make the notion of \textit{safety} rigorous in the context of the dynamical system in \cref{eq:general_dyn}. 
We begin by specifying a set that we wish to render safe:
\begin{align}
   \safeSet = \{\gs \in \gX : h(\gs) \ge 0\} \subset \gX,
   \label{eq:safe_set}
\end{align}
where $h:\gX \to \R$ is a continuously differentiable function. In the case of bipedal walking, safe sets can describe conditions such as admissible torso angles and reasonable foot placement as shown in the first block of \cref{fig:overview}. We assume that the compact set $\safeSet$ is nonempty, has a non-empty interior,
and does not contain isolated fixed-points. We say that $\safeSet$ is \textit{safe} or \textit{forward invariant} if $x(t_0) \in \safeSet$ implies that $x(t) \in \safeSet$ for all $t \ge t_0$. With this, we have the following condition for safety (see \citep{ames_control_2019} for a brief history of this approach):
\begin{definition}[\textit{Control Barrier Function (CBF), \citep{ames2016control}}]
Consider $\safeSet$ as defined in \cref{eq:safe_set} where the continuously differentiable function $h$ has nonvanishing gradients $Dh(\gs) \neq 0$ for all $\bm \gs$ in the boundary of $\safeSet$ defined as $\partial \safeSet = \{\gs \in \gX : h(\gs) = 0\}$. The function $h$ is a \textit{Control Barrier Function} (CBF) for \cref{eq:general_dyn} on $\safeSet$ if there exists $\alpha\in\mathcal{K}_{\infty,e}$ such that for all $\gs\in \safeSet$:
\begin{align}
\label{eqn:CBF}
\dot{h}(\gs) = \frac{\partial h}{\partial \gs}(\gs)\gf(\gs,\gu) \ge -\alpha(h(\gs)).
\end{align}
\end{definition}


A function $\alpha$ is in the family of class-$\mathcal{K}_{\infty, e}$ functions if for all $a<b$,  $\alpha(a) < \alpha(b)$, $\alpha(0) = 0$, $\lim_{a\to\infty} \alpha(a) = \infty$ and $\lim_{a\to-\infty} \alpha(a) = -\infty$. In defining the CBF, we can parameterize the set of all feedback controllers guaranteeing safety as:
\begin{align}
    K_{cbf}(\gs) = \left\{\gu \in \gU : \dot h(\gs, \gu) \ge -\alpha(h(\gs))\right\}.
    \label{eq:k_cbf_set}
\end{align}
Similarly, this notion can be extended to discrete-time dynamical systems via:
\begin{align}
\label{eqn:CBF_disc}
    \Delta h(\bm x_k, \bm u_k)  \triangleq h(\bm x_{k+1}) - h(\bm x_k) \ge -\gamma h(\bm x_k),~~0<\gamma\le 1,
\end{align}
as seen in Figure~\ref{fig:ZDandBarriers}b. This leads to the following necessary and sufficient condition for safety:
\begin{theorem}[\textit{Control Barrier Function Certificates, \citep{ames2016control}}]
Given a feedback controller $\gu=k(\gs)$, the set $\safeSet$ is safe if and only if $\gu(\gs) \in K_{cbf}(\gs)$.
\end{theorem}



==> arXiv/Sections/SimAndExp.tex <==
\vspace{-2 mm }\section{Simulation and Experimental Results}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{Figures/GaitTiles.png}
    \vspace{-20pt}
    \caption{Gait tiles of the neural network encoding the final trained policy running in real time on the AMBER-3M robot. For a video discussing the methodology and summarizing the hardware results, please refer to \citep{video_noauthor_supplementary_nodate}.}
    \label{fig:amber_walking}
\end{figure}
The hardware platform used in this work was the planar underactuated biped AMBER-3M \citep{ambrose_toward_2017}, which has actuators on the hips and knees, and point contact feet. Both in simulation, where the RaiSim \citep{8255551} environment was used, and on hardware, the pipeline went as follows: the zero dynamics coordinate $\bm z$ was estimated, the Neural Network policy $\bm y_d(\bm z;\bm \theta)$ was evaluated, and the desired output values were passed to a PD controller running at 1kHz.
The policy $\bm y_d(\bm z; \bm \theta)$ was randomly initialized and was trained for 1000 epochs. The AdamW optimizer was used in PyTorch \citep{NEURIPS2019_9015} with an initial learning rate of $10^{-2}$, weight decay of $10^{-4}$,  with a learning rate decay schedule at epochs 100, 400, and 800. Initially, the ''gait" had the robots leg flailing randomly in the air, and when integrated resulted in the robot falling over. Once the loss converged, the policy had a loss in the order of $5\times10^{-3}$, and was able to walk stably in the simulation. The neural network ran in closed loop on the hardware platform and was called at approximately 500 Hz to produce desired outputs for the system to track. Unlike simulation, once tested on hardware, the policy resulted in the robot stumbling forward, unable to walk without falling. Data was collected over various trials, after which the methodology proposed in \cref{sec:learn_eps} was used to learn the residual of the model uncertainty, as projected to the zero dynamics space. During this process, Adam and other SGD methods were numerically unstable even with gradient clipping, so Nero \citep{liu_learning_2021} was used instead. 

Once a residual term was learned, a new policy $\bm y_d(\bm z, \bm \theta)$ was trained with the updated dynamics (warm started with the policy from the previous iteration). After convergence, the gait was again tried on hardware. The gait was significantly more stable, and able to walk without assistance; however, the gait was not robust to walking speeds. Therefore, the process was repeated, and again a new policy was learned. When testing that policy, the robot was able to walk on its own, and was robust to different walking speeds. A sample gait is shown on \cref{fig:amber_walking}. The complete code can be found here \citep{git_rodriguez_learning_2021}.






==> arXiv/Sections/WalkingAsBarriers.tex <==
\section{Neural Gaits: Locomotion as a Barrier Satisfiability Problem}
\label{sec:proposed_method}

We now present our Neural Gaits approach, as depicted in \cref{fig:overview}. Instead of taking a controller-design perspective, we will take one of reference trajectory design -- specifically, we fix a controller structure $\bm u(\bm x;\bm \theta)$, which is parameterized by $\bm \theta$ through the definition of $\bm y(\bm x; \bm \theta)$.
Our method relies on the assumption that good walking can be characterized as a forward invariant set.
Thus, the first step of the method requires us to define a set of barrier functions that imply good walking.
In the following discussion, we will only consider barrier functions defined on the zero dynamics surface, i.e. $h:\mathcal{Z}\to\mathbb{R}$ as defined when the error coordinates are zero ($\bm \eta = \bm 0)$.
Importantly, the guarantees made on $\mathcal{Z} \subset \gX$ have relevance to the full state space, as is made precise in Section~\ref{sec:guarantees}.

After constructing a collection of barrier functions, we train a policy $\bm{y_d}$ that ensures the system stays safe by minimizing the violation of the barrier function conditions \eqref{eqn:CBF} and \eqref{eqn:CBF_disc} over regions of the state space.
The resulting policy renders the intersection of the safe set for all barriers forward invariant.
Finally, to mitigate model mismatch, we train a residual term $\varepsilon({\bm z})$ on the zero dynamics.
These corrected zero dynamics are then used to refine the existing policy episodically until the desired walking performance is achieved. 


\subsection{Learning the Policy \texorpdfstring{$\bm{y_d}$}{yd}}

Our learning approach builds upon and unifies two lines of work. 
The first studies how to characterize good walking behavior as set invariance  via a collection of barrier function candidates \citep{ames_first_2017}.
The second studies how to train neural ODEs to satisfy control-theoretic properties such as Lyapunov stability \citep{lyanet}, which we extend to the barrier setting.


\paragraph{Learning in the Zero Dynamics.}
Recall from \cref{sec:prelim:output_and_zdyn} that the error and zero dynamics coordinates are computed from the states using the diffeomorphism $\bm \Phi$, which
only depends on the policy through $\bm \Phi_{\bm \eta}$.
We thus parameterize the policy as a function of the projection of the state onto the zero dynamics manifold and parameters $\bm \theta$, i.e. $\bm{y_d}(\bm x) = \bm{y_d}(\bm \Phi_{\bm z}(\bm x); \bm \theta)$. In other words, $\bm y_d$ only depends on the unactuated degrees of freedom of the system (e.g., the unactuated joint in \cref{fig:hzd_decomposition}) rather than the full state.
Therefore, when there is no error (i.e. $\bm \eta = 0$) we have that $\bm z\in\mathcal{Z}$ with dynamics $\dot{\bm z} = \bm \omega(\bm 0, \bm z; \bm \theta)$.
Note, importantly, that even when the error coordinates are zero, the zero dynamics are still a function of $\bm{y_d}$ and therefore $\bm \theta$. This implies that the zero dynamics are influenced by the parameters of the policy even though the control inputs are not present in $\bm \omega$.



\paragraph{Learning to Satisfy Barrier Conditions.}
Taking inspiration from \citep{hsu2015control} and \citep{ames_first_2017}, we assume that walking can be characterized as set invariance via a collection of barrier function candidates $\mathcal{H} = \{h_i\}_{i=1}^N$ (see \cref{table:barriers} discussed later in \cref{sec:application}).
To each $h_i$, we associate a \textit{region at risk}  $ \overline{\cal{S}}_i \subseteq \cal{Z}$ where the barrier function is enforced. We define a set of neural network parameters that render the region at risk safe under the barrier definition:
\begin{align}
\label{eq:safe_yd_params}
    \bm \Theta_i = \{\bm \theta \in \bm \Theta : \forall_{\bm{z} \in \overline{\cal{S}}_i} \quad \dot h_i(\bm z ; \bm \theta) \ge -\alpha(h_i(\bm z;\bm \theta))\}.
\end{align}
In other words, each $\bm \Theta_i$ corresponds to the set of policy parameters that render the set $\overline{\mathcal{S}}_i$ safe.

Thus, our learning problem is equivalent to finding a set of parameters $\bm \theta \in \bigcap_{i=1}^N \bm \Theta_i$ that render the system safe in all regions at risk.  Similar to the Lyapunov Loss studied in \citep{lyanet}, we introduce the concept of \textit{Barrier Loss} as a learning signal for training:
\begin{definition}[Barrier Loss]
For a set of barrier function candidates $\mathcal{H} = \{h_i\}_{i=1}^N$ and corresponding regions at risk $\overline{\cal{S}}_i \subset \mathcal{Z}$ on the zero dynamics, a Barrier Loss, $\loss: \bm \Theta \to \R_{\geq 0}$, is defined as:
\begin{align}
    \loss(\bm\theta) = \sum_{i=1}^N \int_{\overline{\cal{S}}_i} \max\{0,  - \dot h_i(\bm z ;  \bm \theta) - \alpha(h_i(\bm z;\bm \theta)) \} d\bm{z}. \label{eq:loss}
\end{align}
\vspace{-4mm}
\label{def:loss}
\end{definition}
When a choice of parameters $\bm\theta$ achieves zero Barrier Loss, then the safety of the zero dynamics is guaranteed by satisfying the forward invariance condition of the barrier functions:
\begin{theorem}[Zero Barrier Loss Implies Safety of Zero Dynamics]
\label{thm:zero_barrier_loss}
The zero dynamics is guaranteed to be safe in all its regions at risk 
 if and only if we find a $\bm{\theta}^*$ that attains  $\loss(\bm{\theta}^*) = 0$. 
\end{theorem}
\begin{proof}
Notice that for all $i \in \{1 \ldots N \}$ both $\dot{h}_i$  and $\alpha \circ h_i$ are continuous functions. This implies that for all $\bm z \in \mathcal{Z}$ and $\bm \theta \in \bm \Theta$, $\max\{0,  - \dot h_i(\bm z ;  \bm \theta) - \alpha(h_i(\bm z;\bm \theta)) \}$ is a continuous non-negative real function. It is well known that a continuous non-negative real function will have zero integral if and only if it is the zero function. We specialize this statement for the terms in our loss as follows:
\begingroup\makeatletter\def\f@size{10.2}\check@mathfonts
\begin{align}
    \forall_{\bm z \in \overline{\cal{S}}_i} \max\{0,  - \dot h_i(\bm z ;  \bm \theta) - \alpha(h_i(\bm z;\bm \theta)) \} = 0 \Leftrightarrow \int_{\overline{\cal{S}}_i} \max\{0,  - \dot h_i(\bm z ;  \bm \theta) - \alpha(h_i(\bm z;\bm \theta)) \} d\bm{z} = 0
\end{align}
\endgroup
It is clear that the sum in $\loss(\bm\theta)$ will be zero if an only if each integral term is zero since each integral is a non-negative function. Thus we can conclude that $\loss(\bm\theta^*)=0$  if and only if $$\forall_{i \in \{1 \ldots N \}, \bm z \in \overline{\cal{S}}_i} \max\{0,  - \dot h_i(\bm z ;  \bm \theta^*) - \alpha(h_i(\bm z;  \bm \theta^*)) \} = 0.$$ For any barrier $h_i$ and $\bm z \in \cal{Z}$ you can see that  $\max\{0,  - \dot h_i(\bm z ;  \bm \theta^*) - \alpha(h_i(\bm z;\bm \theta^*)) \} = 0$ implies that: 
\begin{align}
    - \dot h_i(\bm z ;  \bm \theta^*) - \alpha(h_i(\bm z;\bm \theta^*)) \leq 0 \implies
    \dot h_i(\bm z ;  \bm \theta^*) \geq -\alpha(h_i(\bm z;\bm \theta^*)), \nonumber
\end{align}
i.e. 
the safety condition for the barrier is satisfied.
\end{proof}

\subsection{Instantiation for Bipedal Walking}
\label{sec:application}
\cref{table:barriers} describes the barrier functions used in our experiments, which take inspiration from \citep{ames_first_2017}. 
We depict some of these conditions on the robot in \cref{fig:barriers_and_pssf}a.
As all barrier functions $h_i : \mathcal{X} \to \mathbb{R}$ are enforced on the zero dynamics surface, we will write them implicitly as $h_i~\circ~\bm \Phi^{-1}(\bm 0, ~\cdot~;\bm \theta) : \mathcal{Z} \to \R$ for $i \in \{1 \ldots N\}$ with $N=5$ in this instantiation. 
In \cref{table:barriers}, $t_A$ represents the torso angle, and $p_x$ and $p_z$ represent the $x$ and $z$ position of the swing foot, respectively. In addition to continuous time conditions, various conditions needed to be enforced on the guard, namely enforcing the location of the guard, symmetry of the model before and after impact, and a guard mapping condition. 
Interestingly, although these barriers would be relative degree two on the full state dynamics, they are directly enforceable as relative degree one barriers on the zero dynamics. This can be seen by treating $\bm {y_d}$ as the input to the zero dynamics, and observing that the zero dynamics themselves are functions of $\bm {y_d}$.

\begin{table} [b]
\begin{center}
\begin{small}
\begin{tabular}{|c|c|c| }
 \hline
 Torso Angle & $\{\bm z\in \mathcal{Z}_\mathcal{O}\}$ & $-\frac{\pi}{10} \le \theta_t(\bm z) \le 0.05$ \\ 
 \hline
Swing Foot Clearance & $\{\bm z\in \mathcal{Z}_\mathcal{O}\}$ & $0 \le (p_x(\bm z)-c_x)^2 + (p_z(\bm z)-c_z)^2 - r^2 \le 0.3$ \\
 \hline
 Impact Mapping & $\{\bm z\in \mathcal{S}_\epsilon\}$ & $-0.15 \le \Delta(\bm z) + \bm z \le 0.15$ \\
 \hline
 Symmetry & $\{\bm z\in \mathcal{S}_\epsilon\}$ & $\bm y(\bm z) = \bm y(\Delta(\bm z))$\\
 \hline 
 Foot on Guard & $\{\bm z\in \mathcal{S}_\epsilon\}$ & $p_z(\bm z) = 0$ \\
 \hline
\end{tabular}
\end{small}
\caption{Barrier functions used to characterize bipedal walking, and the associated regions at risk in which they are enforced. The first two are enforced over the continuous dynamics, and the bottom three in a buffered region of the guard. The strict equality on symmetry and the foot on guard conditions were also enforced as a training loss. \label{table:barriers}}
\end{center}
\end{table}


Note that these barrier functions $h$ are defined over the space $\mathcal{Z}$, as, given a policy $\bm{y_d}(~\cdot~;\bm{\theta}):\mathcal{Z}\to\mathbb{R}^4$, the mapping $\bm \Phi^{-1}:\mathcal{N}\times\mathcal{Z}\to\pX$ is uniquely defined. 
We take inspiration from reduced order models, and specifically the notion of orbital energy \citep{pratt_derivation_2007} to define a set $\mathcal{Z}_\mathcal{O} \subset \mathcal{Z}$ with reasonably bounded orbital energies as our first region at risk. 
We also define the set $\mathcal{S}_\epsilon \subset \mathcal{Z}_\mathcal{O}$ which contains the part of the guard in  $\mathcal{Z}_\mathcal{O}$ as well as a small region around it where discrete-time guard conditions are enforced. We learn policies that satisfy the barrier conditions on these regions of the zero dynamics by penalizing the violation of the constraints shown in \cref{table:barriers}. Notice that penalizing guard constraints over a region results in policies that are robust to impact modeling error since the policy must be prepared to change stance foot at any point in $\mathcal{S}_\epsilon$ rather than just the guard $\mathcal{S}$.

\textbf{Learning Optimization Details.}
Evaluating the Barrier Loss in \cref{eq:loss} requires solving an integral that is in general intractable.
Instead, we use Monte Carlo sampling to approximate the integral.
Since our approach follows Algorithm 1 of \citep{lyanet} we refer to it for more details while noting that we optimize for the Barrier Loss rather than the Lyapunov Loss.
A key ingredient in the Monte Carlo sampling approach in \citep{lyanet} is defining a compact support set to sample from (i.e., where the barrier condition should be satisfied). In our work this compact support set directly corresponds to the region at risk for each barrier condition.
\vspace{-2mm}
\subsection{Learning the Residual Zero Dynamics \texorpdfstring{$\bm \varepsilon(\bm z)$}{varepsilon(z)}}
\label{sec:learn_eps}
As outlined in \cref{fig:overview}, we can improve upon the nominal zero dynamics model by collecting trajectories of the robot executing the resulting policy in hardware.  We can then use those trajectories to learn a residual error term on the zero dynamics $\hat{\dot{\bm z}} = \omega(0, \bm z ; \bm \theta) + \varepsilon(\bm z)$ where $\varepsilon$ is the learned residual term. We model this residual term using Neural ODEs \citep{chen_neural_2019}, which are naturally compatible with our policy learning approach. We can iterate this process multiple times, alternating between learning $\bm \theta$ and $\varepsilon$ until the resulting policy achieves the desired behavior.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{Figures/BarriersAndPssf_V2.pdf}
    \vspace{-20pt}
    \caption{\textbf{a)} A depiction of the barrier functions used to enforce walking as set invariance. On the left are the two continuous time barrier conditions, and on the right the three barrier conditions enforced at the guard. The red dot on the foot indicates the stance foot, and \textbf{b)} The safe set on the zero dynamics $\mathcal{C}_{\mathcal{Z}}$, as certified by the proposed learning method, and the combined safe set $\mathcal{C}_{\sigma}$, and described in Theorem 5.}
    \label{fig:barriers_and_pssf}
\end{figure}
\vspace{-2mm}
\subsection{Providing Guarantees in the Full State Space}
\label{sec:guarantees}
Assuming a controller which exponentially converges the outputs $\bm y(\bm x)$, for example a feedback linearizing or control Lyapunov function based controller, the converse Lyapunov theorem allows us to construct a Lyapunov function $V_{\bm\eta}:\mathcal{N}\to\mathbb{R}$ verifying the exponential convergence of the outputs. Along with a certificate of safety $h_Z:\mathcal{Z} \to \mathbb{R}$ on the zero dynamics space, we can construct a set in the combined space $\mathcal{N}\times \mathcal{Z}$ which is safe, and has a barrier function certificate. This is described in the following theorem.

\begin{theorem}%
\label{thm:zero_dyn_barriers_pssf}
Let $V_{\bm \eta}=\bm \eta^\top\bm P\bm \eta:\mathcal{N}\to\mathbb{R}$ be an exponential control Lyapunov function for the output dynamics with $\dot V_{\bm \eta} \le -\gamma V_{\bm \eta}$ and $h_Z:\mathcal{Z}\to\mathbb{R}$ be a barrier function on the zero dynamics with safe set $\mathcal{C}_\mathcal{Z}$. Then, there exists a constant $\sigma\ge 0$ and $c\ge 0$ such that if $\dot h_Z(z) \ge -\alpha h_Z(z) + c$ with $\alpha\le \frac{\gamma}{2}$, the barrier function $ h (\bm \eta, \bm z) =  h_Z(\bm z) - \sigma V_{\bm \eta}(\bm \eta)$ is safe with set $\mathcal{C}_\sigma$.%

\end{theorem}
\begin{proof}
First note that the derivative of the function is given by:
\begin{align}
    \dot{ h} &= \frac{\partial  h_Z}{\partial \bm z} (\bm z) \bm w(\bm\eta , \bm z) - \sigma\dot V_{\bm \eta}(\bm \eta) \notag \\
    &\ge -\alpha  h_Z(\bm z)+c - \left|\frac{\partial  h_Z}{\partial \bm z} (\bm z) \left(\bm w(\bm\eta , \bm z)-\bm w(0 , \bm z)\right)\right| + \sigma\gamma V_{\bm \eta}(\bm \eta) \notag \\
    &\ge -\alpha  h(\bm \eta, \bm z) + c- L_{ h_Z}L_{\bm \omega_{\bm \eta}}\|\bm\eta\|_2+ \frac{\sigma\gamma}{2} \lambda_{min}(\bm P)\|\bm \eta\|_2^2, \label{eqn:RobustSafeSet}
\end{align}
where the third line follows from Cauchy Schwartz, the fact that $ h_Z$ and $\bm \omega(\bm \eta, \bm z)$ are locally Lipschitz with Lipschitz constants $L_{ h_Z}$ and $L_{\bm \omega_{\bm \eta}}$, respectively, converse Lyapunov, and the assumption that $\alpha\le \frac{\gamma}{2}$. Taking $\beta_1 = L_{ h_Z}L_{\bm \omega_{\bm \eta}}$, and $\beta_2 = \frac{\gamma}{2} \lambda_{min}(\bm P)$, we observe that $-\beta_1\|\bm\eta\|_2 + \sigma \beta_2\|\bm \eta\|_2^2 \ge -\frac{\beta_2^2}{4\sigma\beta_3}\triangleq c$. By taking $c$ defined as such, we achieve the desired result.
\end{proof}

The above theorem motivates the perspective of this work: satisfying barrier function certificates in the zero dynamics enables reasoning about safe sets in the complete state space. Note that the hybrid case is not addressed here, and is an interesting direction for future theoretical work. 

==> main_backup.tex <==
% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}
% \IEEEoverridecommandlockouts    
% \usepackage{times}

% % numbers option provides compact numerical references in the text. 
% % \usepackage[numbers]{natbib}
% \usepackage{multicol}
% \usepackage[bookmarks=true]{hyperref}

% % The following packages will be automatically loaded:
% % amsmath, amssymb, natbib, graphicx, url, algorithm2e

% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{graphicx}
% \usepackage{epstopdf}
% \usepackage{mathtools}
% \usepackage{dsfont}
% \usepackage{tikz}
% \usepackage{siunitx}
% \usepackage{hyperref}
% \usepackage[font=footnotesize]{caption}
% % \usepackage{floatrow}
% \usepackage[noabbrev,capitalize]{cleveref}
% \usepackage{balance}    % have even columns on last page
% \usepackage{xcolor}
% \usepackage{tcolorbox}
% % \usepackage{algorithm}
% % \usepackage{algpseudocode}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% % \usepackage{algorithm2e}
% \usepackage{mathtools}
% \usepackage{dsfont}
% \usepackage{mathrsfs}
% % \usepackage[noadjust]{cite} % multiple citations are combined
% \usepackage{stmaryrd}
% \usepackage{placeins}
% \usepackage{upgreek}
% \usepackage{wrapfig}
% \usepackage{bm}
% \usepackage{cases}
% \usepackage{bbm}
% \usepackage{noel}

% % \usepackage[backend=biber, natbib=true, style=apa, hyperref=true, firstinits=true, maxcitenames=1, parentracker=true, maxbibnames=99]{biblatex}
% % \addbibresource{./references.bib}

% \DeclareMathOperator*{\argmin}{argmin}
% \DeclareMathOperator*{\argmax}{argmax}   

% % \title{\LARGE \bf Constructive Feedback Controllers for Underactuated Systems \\ via Zero Dynamics Policies}
% \title{\LARGE \bf Constructive Nonlinear Control of Underactuated Systems \\ via Zero Dynamics Policies}

% \begin{document}
% \author{William Compton$^*$, Ivan Dario Jimenez Rodriguez$^*$, Noel Csomay-Shanklin$^*$, \\Yisong Yue, Aaron D. Ames%
% \thanks{This research is supported by Technology Innovation Institute (TII).}
% \thanks{$^*$denotes equal contribution. Authors are with the Department of Computing and Mathematical Sciences, California Institute of Technology,
% Pasadena, CA 91125. This research was supported by NSF Graduate Research Fellowship No. DGE‐1745301, AeroVironment, NSF Grant No. 1918655 and Raytheon, Beyond Limits, JPL RTD 1643049.}
% }

% \maketitle

% % Stabilizing underactuated systems remains a challenging task in control theory due to the existence of fundamental limits on how the control input can affect the system dynamics. The decomposition of such systems into actuated and unactuated states, namely output and zero dynamics coordinates, has provided useful insight into the underlying structure that exists, but has yet to result in constructive ways to stabilize such systems. 
% % Despite these fundamental limits, modern control approaches such as Model Predictive Control (MPC) and Reinforcement Learning (RL) have demonstrated a surprising ability to stabilize such systems, but have largely overlooked the underlying structure that is present. 
% % The goal of this work is to reconcile these two perspectives by analyzing the way in which MPC and RL are able to stabilize these underactuated states, and in doing so developing a canonical, low-dimensional action space through which learned policies can stabilize the full system state. Specifically, we formalize the idea of zero dynamics policies -- policies which map from the underactuated states of a system to the output space -- and provide conditions under which stabilization of the full system state can be achieved.

% \vspace{-6mm}
% \begin{abstract}%
% Stabilizing underactuated systems is an inherently challenging control task due to fundamental limits on how the control input affects the passive system dynamics.
% Despite these challenges, horizon-based methods can successfully stabilize these systems but largely overlook the structure of underactuation. 
% The decomposition of underactuated systems into actuated (output) and passive (zero) dynamics coordinates has provided useful insight into the underlying structure of systems of this form.
% In this work, we combine the insight into the zero dynamics structure with the constructive stability of horizon based planners to formalize the idea of \emph{Zero Dynamics Policies (ZDPs)}---a learned mapping from the passive coordinates to the actuated coordinates. 
% Specifically, we show that a ZDP exists in a neighborhood of the origin, and prove that combining output feedback with a ZDP results in stability of the underactuated system.  We demonstrate that such a paradigm can be used to stabilize the canonical underactued system of the cartpole.
% \end{abstract}

% \IEEEpeerreviewmaketitle

% % \begin{keywords}%
% %   bipedal locomotion, zero dynamics, safety, robotics
% % \end{keywords}

% % \blfootnote{$^*$ These authors contributed equally to this work.}
% % \vspace{-4mm}
% % \section{Introduction}
% % % \input{Sections/Introduction}
% % \input{Sections/Introduction_v2}

% \section{Introduction}
% % the ability to arbitrarily shape a vector field which many of
% Feedback is the cornerstone of control theory.
% % Feedback is the fundamental tenet upon which the field of control theory is built. 
% Constructive feedback controllers for nonlinear systems -- e.g. input-output linearization \cite{sastry_linearization_1999} and control Lyapunov functions \cite{sontag_control-lyapunov_1999} -- rely on the ability to arbitrarily shape a system's vector field. 
% \textit{Underactuated} systems -- e.g. legged robots, dexterous manipulators, and systems with strict actuator limits --  cannot actuate all degrees of freedom, which results in vector fields that cannot be arbitrarily shaped.
% % Underactuation, however, fatally undermines many of the assumptions that constructive methods of designing feedback controllers for nonlinear systems rely on. For example, the -- 
% Importantly, restricted actuation authority does not imply a loss of stabilizability; achieving stable behaviors, however, requires careful coordination of the actuated degrees of freedom. 

% Our approach leverages \textit{Zero dynamics}: a powerful tool for analyzing underactuated systems  which considers the residual dynamics when all outputs have been zeroed \cite{isidori_elementary_1995}.
% Traditional Zero Dynamics approaches, craft output coordinates that induce induced zero dynamics which are then algebraically checked for stability.
% Underactuation forces this guess-and-check approach because of how challenging it is to find feedback linearizable output coordinates which span the complete state space \cite{bedrossian_nonlinear_nodate}.
% Even if these output coordinates can be found, verifying the algebraic stability conditons can be difficult.
% Instead our approach explicitly uses outputs as learnable design variables, enabling stable zero dynamics by construction.
% Using, output tracking for stable convergence to the surface defined by these learnable outputs results in stability of the overall system.

% % \textit{Zero dynamics} -- a powerful tool for analyzing underactuated systems -- considers the residual dynamics when all outputs have been zeroed \cite{isidori_elementary_1995}.
% % Underactuation makes it challenging if not impossible to find feedback linearizable output coordinates which span the complete state space \cite{bedrossian_nonlinear_nodate}. 
% % Even if such coordinates exist, verifying the algebraic conditions required to identify them is difficult.
% % Traditionally, this approach involves first designing an output and subsequently analyzing the induced zero dynamics.
% % This sequential process, however, removes the degrees of freedom that output shaping provides from the design process, relying on clever output design to result in stable zero dynamics. 
% % Our approach diverges from this tradition by explicitly leveraging the outputs as design variables, allowing us to induce stable zero dynamics by construction.
% % We parameterize the surface in such a way such that, once identified, output tracking tools can be used to stabilize the surface resulting in composite stability of the overall system. 

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/M_characteristics.png}
%     \caption{The two conditions required of the zeroing manifold: a) invariance under stabilizing control, and b) stable zero dynamics.}
%     \label{fig:enter-label}
%     \vspace{-6mm}
% \end{figure}

% This work continues the line of research studying stabilization of nonminimum phase systems \cite{devasia_nonlinear_1996, tomlin_output_1995, isidori_output_1990} and extends work proposing the design of a stabilizing zero dynamics manifold in the context of Hybrid Zero Dynamics for stable walking behavior \cite{westervelt_hybrid_2003}. 
% Optimal control has also proven to be a useful and constructive tool which is able to stabilize systems despite their underactuation. There are two main methods of solving optimal control problems: either solving directly for a feedback strategy by approximating the value function, or applying a receding horizon approach via MPC. Both of these approaches suffer from dimensionality issues, as the total state space may be large for systems of interest. In this work, we aim to leverage the algorithmic stabilizing capability of optimal control with the dimension reduction provided by the zero dynamics analysis. 


% % Model predictive control is another technique which has demonstrated significant success in the context of stabilizing underactuated systems.

% % Despite the impressive results in the field of robotics for the control of underactuated systems, our fundamental understanding of the interaction between the actuators and the resulting system dynamics, and therefore ability to design appropriate feedback controllers, remains limited.

% To this end, we propose a mapping from the underactuated coordinates to the actuated coordinates as a means for stabilizing underactuated systems. This structure is inspired by many successful results in legged robotics \red{cite}, which often apply feedback on the actuated subspace as a function of the unactuated one. A notion of zero dynamics policies was explored in \cite{rodriguez_neural_2022}, wherein walking for a planar biped was generated by enforcing barrier function certificates. In this work, we: 1) extend zero dynamics policies to continuous time systems, 2) show that this mapping is well defined for controllable nonlinear systems, 3) prove that output tracking results in stability of the overall system, and 4) give constructive methods of designing this surface via optimal control. Finally, we apply the proposed Zero Dynamics Policy method to control a nonlinear cart pole and demonstrate a larger region of attraction than traditional control methods.

% % In different control contexts, outputs can have varied interpretations, including sensor measurements in the context of observability; we will instead be interested in outputs insofar as we can constructively use control to manipulate their behavior.

% % If the dynamics in \eqref{eqn:} satisfy a controllability and involutivity property with respect to the vector fields $\b f$ and $\b g$, it is possible to generate an output which full-state feedback linearize the system dynamics \cite{isidori_elementary_1995}. Unfortunately, underactuated systems often do not satisfy these requirements \cite{murray_cart_pole_not_involutive}, and therefore require careful coordination of the actuated coordinates to induce stability on the entire system state. 

% %%%%%%%%%% YISONG COMMENTS %%%%%%%%%%%%
% % Discuss what you are implying by constructive
% % 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % To combat dimensionality and issues with online computational overhead, we will develop a method which exploits the aforementioned output and zeroing structure present in \eqref{eq:zd}. Specifically, we propose finding a function $\func:Z\to\mathcal{N}$ mapping between the underactuated and actuated coordinates, which draws inspiration from many successful results in robotics \red{raibert, centroidal MPC, backstepping, sliding mode control}

% % Random one sentence claims:
% % \begin{itemize}
%     % \item Importantly, restricted actuation authority does not imply a loss of stabilizability; however, achieving stable behaviors requires careful coordination of the actuated degrees of freedom. 
%     % \item 
%     % \item In contrast to the typical perspective of outputs as observers \cite{kalman_new_1960}, we will instead be interested in outputs for which there exist constructive stabilization techniques.
%     % \item For underactuated robotic systems, it is often challenging if not impossible to find output coordinates which span the complete state space and which can be feedback linearized \cite{bedrossian_nonlinear_nodate}. Even if such coordinates exist, verifying the algebraic conditions required to identify them is difficult. 
%     % In light of this, we will focus on producing coordinates which are of valid relative degree, and which when tracked will result in stability of the complete system.\cite{isidori_elementary_1995-1}. In light of this, we will focus on producing coordinates which are of valid relative degree, and which when tracked will result in stability of the complete system.
%     % \item There exist conditions on the existence of outputs which render the system full-state feedback linearizeable, and therefore do not have zero dynamics \ref{sastry_linearization_1999}. These conditions are difficult to verify, but are in general not satisfied for many control systems of interest.
%     % \item For underactuated systems, the rank deficiency of the matrix $\b B$ often implies a lack of involutivity of the distribution $\b \Delta(\b x)$, and therefore an inability to choose any output $\b y$ which results in full state feedback linearizeability.
%     % \item The main objective of this work is to construct a feedback controller $\b u(\b x)$ which renders an equilibrium point $\b x^*$ exponentially stable for the underactuated system \eqref{eq:robot_dynamics}. As asymptotic stability is a necessary condition for optimality\footnote{Under the mild assumption that the system is observable under the state stage cost.}\cite{liberzon_calculus_2012}, one such controller is the solution to the infinite time optimal control problem
%     % \item 
    
%     % To combat dimensionality and issues with online computational overhead, we will develop a method which exploits the aforementioned output and zeroing structure present in \eqref{eq:zd}. Specifically, we propose finding a function $\func:Z\to\mathcal{N}$ mapping between the underactuated and actuated coordinates, which draws inspiration from many successful results in robotics \red{raibert, centroidal MPC, backstepping, sliding mode control}
% % \end{itemize}

% % We show the following:
% % \begin{itemize}
%     % \item We focus on the design of feedback policies for underactuated systems
%     % \item We propose a mapping from the underactuated coordinates to the actuated coordinates and prove that driving the error to zero results in composite stability of the overall system. This takes inspiration from many results in robotics
%     % \item For this mapping to be well defined, it must define a attractive and invariant submanifold of the state space
%     % \item We prove that for systems which admit an LQR solution, this manifold exists and is well defined in a neighborhood of the origin.
%     % \item We show that if the manifold is both forward invariant and has stable autonomous dyanmics, the entire system sis stabilizeable by converging to the manifold
%     % \item the manifold exists in the actuator null space, termed the unactuated coordinates
%     % \item We give constructive methods of finding this manifold using optimal control and machine learning
% % \end{itemize}


% % A powerful tool to analyze underactuated systems, or more generally systems which are not full state feedback linearizeable, has been through their \textit{zero dynamics}, i.e. the residual dynamics when all available outputs have been zeroed. Historically, this process begins by defining an output and analyzing the residual dynamics once the outputs have been zeroed. This process, however, removes the degrees of freedom from the design process which may be used precisely to stabilize the resulting zero dynamics. Instead, in our approach, we leverage the outputs as design variables, and use stability criteria to define what form the outputs should take such that the zeroing manifold is stable. We parameterize the surface in a way such that once identified, output tracking tools can be used to stabilize the surface, giving composite stability of the overall system by construction. 

% % Theoretical statements we would like to make:
% % \begin{itemize}
%     % \item There are a whole class of controllers which stabilize the outputs (as long as they are properly designed). Choose your favorite.
%     % \item the level set of $\eta - \psi(z)$ defines a manifold under certain assumptions on $\psi$. conditions on the outputs impose conditions on $\psi$.
%     % \item If this manifold is invariant and stable (given a feedback controller the returns the feedforward input, these are conditions only on $\psi$), then we have composite stability.
%     % \item This manifold exists locally, i.e. there exists a psi that satisfies the above conditions around the origin (LQR). This can be done in two parts, i) it exists for the linearization, ii) the linearization is valid for the nonlinear system.
%     % \item Optimal controllers are stabilizing. 
%     % \item There is a condition, which if satisfied results in the invariance of the manifold. The optimal controllers satisfy this condition (locally).
%     % \item Result: We can structure a learning problem for the cart pole and acrobot. 
% % \end{itemize}

% % The theory of zero dynamics has been 


% % Taking inspiration from linear systems, we know that unstable zeros induce fundamental limits on performance, but do not result in a loss of stabilizeability.

% \clearpage




% \section{Preliminaries}

% \begin{comment}
%     There exist conditions on the existence of outputs which render the system full-state feedback linearizeable, and therefore do not have zero dynamics \ref{sastry_linearization_1999}. These conditions are difficult to verify, but are in general not satisfied for many control systems of interest.

%     For underactuated systems, the rank deficiency of the matrix $\b B$ implies a lack of involutivity of the distribution $\b \Delta(\b x)$, and therefore an inability to choose any output $\b y$ which results in full state feedback linearizeability.
% \end{comment}

% We begin a review of nonlinear control by considering the following nonlinear control-affine system:
% \begin{align} \label{eqn:affine_dyn}
%     \dot{\b{\eta}} &= \begin{bmatrix} \b 0&\b I\\0&\b{0}^\top\end{bmatrix}\b \eta+\begin{bmatrix}\b 0\\ f(\b{\eta}, \b z) \end{bmatrix}+\begin{bmatrix} \b 0\\ g(\b{\eta}, \b z)\end{bmatrix}u \\
%     \dot{\b z} &= \b \omega(\b \eta, \b z)
% \end{align}
% % \begin{align} \label{eqn:affine_dyn}
% %     \dot \eta_i &= \eta_{i+1}, ~~~ i = 1,\ldots, p-1 \\
% %     \dot \eta_p &= f(\b \eta, \b z) + g(\b\eta, \b z) u \\
% %     \dot{\b z} &= \b\omega(\b\eta, \b z)
% %     % \dot{\b{\eta}} &=
% %     % \underbrace{\begin{bmatrix} \b 0&\b I\\0&\b{0}^\top\\ \b 0 & \b 0\end{bmatrix}\b \eta+\begin{bmatrix}\b 0\\ f(\b{\eta}, \b z) \end{bmatrix}}_{ \b{f}(\b{\eta}, \b z)}+\underbrace{\begin{bmatrix} \b 0\\ g(\b{\eta}, \b z)\end{bmatrix}}_{\b{g}(\b{\eta}, \b z)}u \\
% %     % \dot{\b z} &= \b \omega(\b \eta, \b z)
% % \end{align}
% with actuated state $\b \eta\in N\subset \R^{\nn}$, unactuated state $\b z \in Z \subset \R^{\nz}$, input $u \in \R$, and functions $\b f:N\times Z\to \R,  \b g:N\times Z\to \R$, and $\b \omega: N\times Z \to \R^{\nz}$ assumed to be continuously differentiable on the domain of their arguments. Furthermore, we denote the complete state by $\b x =(\b \eta, \b z) \in \mathcal{X} \triangleq N\times Z \subset\R^n$, where $n = \nn + \nz$. For the ensuing discussion, we assume the following:
% \begin{assumption}
%     The functions $f(\b 0, \b 0) = 0$ and $\b\omega(\b 0, \b 0) = \b 0$, and $g(\b \eta, \b z)\ne 0$ for all $(\b \eta, \b z) \in N\times Z$.
% \end{assumption}
% \noindent
% This assumes that the origin is an equilibrium point of the system dynamics and that we never lose actuation authority over the actuated coordinates. 
% Note that although we consider single input, single output systems for clarity of exposition, the results extend to the multiple-input, multiple-output setting under similar assumptions on the invertibility of $g$.
% % The structure of having an integrator on the actuated coordinates and no control input on the underactuated coordinates is common in robotic systems. 
% % This assumption is equivalent to the system \eqref{eqn:affine_dyn} having a relative degree \cite{isidori1995nonlinear}.

% \subsection{Feedback Linearization}

% The assumption that $g(\b \eta, \b z) \ne 0$ allows us to define the pre-feedback controller $k_{\textrm{fbl}}(\b \eta, \b z, v): N \times Z \times \R \to \R$ as:
% \begin{align*}
%     k_{\textrm{fbl}}(\b \eta, \b z, v) \triangleq g(\b \eta, \b z)^{-1}(-f(\b\eta, \b z) + v),
% \end{align*}
% for an auxiliary input $v \in \R.$ This yields the following closed loop actuated dynamics:
% \begin{align*}
%     \dot{\b \eta} = \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 & \b 0 \end{bmatrix}}_{\triangleq \b F}\b \eta + \underbrace{\begin{bmatrix}\b 0 \\ 1\end{bmatrix}}_{\triangleq \b G} v,
% \end{align*}
% with $\b F \in \R^{\nn \times \nn}$ and $\b G\in \R^{\nn}$. 
% For convenience, define:
% \begin{align}
%     \label{eqn:pre_feedback}
%     \b f(\b x) &\triangleq \begin{bmatrix}\b F \b\eta\\\b\omega(\b \eta, \b z)\end{bmatrix},\ \ \ \ \ 
%     \b g(\b x) \triangleq \begin{bmatrix}\b G\\\b 0\end{bmatrix},
% \end{align} as the complete closed loop system dynamics. The goal of this work will be to stabilize system \eqref{eqn:affine_dyn} to an equilibrium point $\b x^*$, which we take without loss of generality to be the origin.
% We will specifically by interested in achieving this goal in the case that $\b \omega$ is unstable, which will require careful coordination of the $\b \eta$ coordinates.

% Many constructive stabilization techniques for nonlinear systems revolve around output stabilization \cite{sastry_linearization_1999}. Let $y:\mathcal{X}\to \R$ denote such an output. 
%  In order for the evolution of this output to be impacted by a controller, the input $u$ must appear in a derivative of the output in a meaningful way. Consider a time derivative of the output:
% \begin{align*}
%     \dot {y}(\b x) = \underbrace{\frac{\partial y}{\partial \b x}\b f(\b x)}_{L_\b f y(\b x)} + \underbrace{\frac{\partial y}{\partial \b x}\b g(\b x)}_{L_\b g y(\b x)} u 
% \end{align*}
% where $L_\b {f} y:\mathcal{X} \to \R$ and $L_\b {g} y:\mathcal{X} \to \R$ are the \textit{Lie derivatives} of the output $y$ with respect to the vector fields $\b f$ and $\b g$, respectively. If $L_\b g y(\b x) \equiv 0$, we can attempt to continue differentiating until a higher derivative is not:
% \begin{align*}
%     {y}^{(r)}(\b x) &= L_\b f^r(\b x) + L_\b gL_\b f^{r-1}(\b x)  u.
% \end{align*}
% Differentiating the output until the input appears is captured in the following notion of strict relative degree:
% \begin{definition}
%     \cite{sastry_linearization_1999} \label{def:rel_deg}
%     An output $y :\mathcal{X} \to \R$ for the system \eqref{eqn:affine_dyn} is said to have relative degree $r\in\mathbb{Z}_{+}$ at $\b x_0$ if:
%     \begin{align*}
%         L_{\b g}L_{\b f}^k y(\b x) \equiv 0,\ \ \ \ 0\le k\le r-2
%     \end{align*}
%     and $L_\b g L_\b f^{r-1} y(\b x_0) \neq 0$.
% \end{definition}

% Given an output of relative degree $r \in \mathbb{N}$, consider the mapping $\b \Phi_{\b e}:\mathcal{X}\to \mathcal{E}\triangleq\R^r$, defined as:
% \begin{align}
%     \b \Phi_{\b e}(\b x) \triangleq \begin{bmatrix}
%         y(\b x) & \dot{y}(\b x) & \cdots & y^{r}(\b x)
%     \end{bmatrix}^\top . \label{eq:error}
% \end{align}
% We will subsequently take $\b e = \b\Phi_{\b e}(\b x)\in\mathcal{E}$ to represent coordinates in the error space. 


% \subsection{Control Lyapunov Functions} 

% Valid relative degree allows the constructive synthesis of controllers which exponentially stabilizes the outputs. 

% \begin{definition}
%     The signal $\b e(t)$ is \textit{exponentially stable} if there exists $\delta, M, \lambda > 0$ such that:
% \begin{align*}
%  \|\b e_0\| \leq \delta \quad \implies \quad    \|\b e(t)\| \leq M e^{-\lambda t} \|\b e_0\|.
% \end{align*}
% \end{definition}

% Lyapunov theory \cite{sontag1989universal} states that exponential stability is one-to-one with the existence of a control Lyapunov function (CLF)
% % The power of Lyapunov theory is 
% % A condition which is often verified by construction of an exponential Lyapunov function 
% $V: \mathcal{E} \to \R$ satisfying:
% \begin{align}
%     k_1\|\b e\|^2 \leq V(\b e) &\le k_2 \|\b e\|^2 \nonumber\\
%     \inf_u \dot{V}(\b x, u) &\le -k_3 V(\b e). \label{eqn:lyap}
% \end{align}
% for $k_i > 0$. We define $\mathcal{K} = \{ k(\b x) ~\vert~ \dot{V}(\b x, k(\b x)) \leq -k_3 V(\b e)\}$ to be the set of all exponentially stabilizing feedback controllers, which is nonempty under valid relative degree \cite{ames2014rapidly}.

% We will be interested in outputs of the form $y(\eta_1, \b z)$; therefore, the following assumption is necessary to ensure that the output maintains relative degree $\nn$:
% \begin{assumption}
%     \label{ass:rel_deg}
%     We have that $\frac{d \b \omega}{d \eta_i} = \b 0$ for all $i = 3,\ldots,\nn$.
% \end{assumption}
% This is satisfied for $\nn \leq 2$, as is common for robotic systems.
% Once the outputs are zeroed, the remaining states evolve on a manifold, motivating the following discussion.
% % We are interested analyzing the dynamics of the system once the error has be zeroed. The remaining dynamics evolve on a manifold, motivating the following discussion.

% \subsection{Manifolds and Control Invariance}

% Consider a differentiable function $\b h:\mathcal{X} \to \R^p$ with $\b 0$ a regular value, i.e. $D\b h(\b 0)$ is full rank. Then, we have that $\mathcal{M}\triangleq \{\b x~|~\b h(\b x) = \b 0 \}$ defines a $p$-dimensional embedded submanifold of $\mathcal{X}$ \cite{spivak_calculus_2018}. Associated with such a manifold is the notion of a tangent space.  Since the manifolds being considered are 0-level sets of a function $h$, a vector $\b v\in \R^n$ is a \textit{tangent vector} to a manifold $\mathcal{M}$ at the point $\b x \in \mathcal{M}$, denoted as $\b v\in \mathsf{T}_{\b x}\mathcal{M}$, if:   
%     \begin{align*}
%         \frac{\partial \b h}{\partial \b x}^\top \b v = \b 0.
%     \end{align*}
% % \begin{definition}
% %     A vector $\b v\in \R^n$ is a \textit{tangent vector} to a manifold $\mathcal{M}$ at the point $\b x \in \mathcal{M}$, denoted as $\b v\in \mathsf{T}_{\b x}\mathcal{M}$, if:   
% %     \begin{align*}
% %         \frac{\partial \b h}{\partial \b x}^\top \b v = \b 0.
% %     \end{align*}
% % \end{definition}
% This aligns with the classical notions of tangent vectors as the gradient field of a function provides a basis for the annihilator of its \textit{tangent space}, the span of all tangent vectors at a point.
% % and the \textit{tangent bundle} is then taken to be the disjoint union of all tangent spaces of the manifold $\mathcal{M}$.
% %

% A key property will be the notion of controlled invariance for such a manifold, defined as:
% \begin{definition}
%     A manifold $\mathcal{M}$ is \textit{controlled invariant} under dynamics \eqref{eqn:pre_feedback} if for all $\b x \in \mathcal{X}$ there exists a $u\in \R$ such that:
%     \begin{equation*}
%         \b f(\b x) + \b g(\b x) u \in \mathsf T_{\b x} \mathcal{M}
%     \end{equation*}
% \end{definition}
% This states that the vector field associated with the dynamics must lie in the tangent space of the manifold. Our proposed method aims to find controlled invariant manifolds with exponentially stable dynamics. 

% \section{Zero Dynamics Policies}

% We propose a differentiable mapping $\b\psi: Z \rightarrow \mathcal{N}$, which maps from the underactuated states $\b z$ to desired locations for the actuated states $\b \eta$. This is motivated by several results in robotics, such as the Raibert Heuristic, which maps a walking robot's center of mass (unactuated) to desired foot positions (actuated). The mapping $\b \psi$ induces a $\nz$-dimensional submanifold of $\mathcal{X}$ via the zero level set of the function $\b h(\b \eta, \b z) \triangleq \b \eta - \b \psi(\b z)$:
% \begin{equation} \label{eq:zdp_manifold}
%     \mathcal{M}_{\b \psi} \triangleq \{ (\b \eta, \b z) \in \mathcal{N} \times Z \ \vert \ \b h(\b\eta, \b z) = \b 0\},
% \end{equation}
% as $D\b h = [\b I~\star]$ is full rank. With this, we can now introduce the notion of \textit{zero dynamics}:

% \begin{definition}
%     The \textit{zero dynamics} associated with a controlled invariant manifold $\mathcal{M}_{\b \psi}$ are given by:
%     \begin{align*}
%         \dot{\b z} = \b\omega(\b\psi(\b z), \b z).
%     \end{align*}
% \end{definition}


% \subsection{Stabilizing Zero Dynamics Policies}


% If the zero dynamics are exponentially stable, we will show that stabilizing $\mathcal{M}_{\b \psi}$ stabilizes the whole system. To this end, we propose the following output:
% \begin{align}\label{eqn:out}
%     y = \eta_1 - \psi_1(\b z),
% \end{align}
% % with the goal that stabilizing this output will stabilize $\mathcal{M}_{\b \psi}$. 
% where $(\cdot)_i$ indicates the $i^{\textrm{th}}$ index.
% We begin by stating a condition for the relative degree of \eqref{eqn:out}:
% \begin{lemma} \label{lem:zdp_invariance}
%     The output $y(\b x) = \eta_1 - \psi_1(\b z)$ has valid relative degree $\gamma$ if an only if $\frac{d\psi_1}{d z}\frac{\partial \b\omega}{\partial \eta_2} \ne 1$.
%     % Consider a controlled invariant manifold defined as in \eqref{eq:zdp_manifold}. If the output $y = \eta_1 - \psi_1(\b z)$ has valid relative degree, then holding $y = \dot{y} = \b 0$ renders $\mathcal{M}$ invariant.
% \end{lemma}
% \begin{proof}
%     Taking derivatives until the input appears yields:
%     \begin{align}
%         % y &= \eta_1 - \psi_1(\b z) \nonumber \\
%         \dot{y} &= \eta_2 - \frac{d\psi_1}{d \b z} \b \omega(\b \eta_{1:2}, \b z)\nonumber \\
%         % \ddot{y} &= \left(1 - \frac{d\psi_1}{d \b z} \frac{d \b \omega}{d \eta_2} \right) \eta_3 + M_2(\eta_{1:2}, \b z) \nonumber\\
%         % &\vdots \nonumber\\ 
%         y^{(i)} &= \left(1 - \frac{d\psi_1}{d \b z} \frac{d \b \omega}{d \eta_2} \right) \eta_{i+1} + W_i(\b \eta_{1:i}, \b z), \label{eqn:output_dot}\\ 
%         % &\vdots \nonumber\\ 
%         y^{(\gamma)} &= \left(1 - \frac{d\psi_1}{d \b z} \frac{d \b \omega}{d \eta_2} \right) u + W_{\gamma}(\b \eta, \b z)\nonumber 
%     \end{align}
%     for $i=2,\ldots,\gamma-1$ and where $W_i: N \times Z \to \R$ is introduced to hold additional terms for each derivative
%     % , keeping track of which coordinates are involved, 
%     , and $\b \eta_{i:j} = [\eta_i \ \ldots \ \eta_j]^\top$.
%     % , and \eqref{eqn:yi} holds for $i = 2, \hdots, \gamma - 1$. 
%     As $u$ does not appear until $y^{(\gamma)}$, we have that $L_{\b g} L_{\b f}^i y \equiv 0$ for $i = 0, \ldots, \gamma - 2$, and $L_{\b g} L_{\b f}^i y = 1 - \frac{d\psi_1}{d \b z} \frac{d \b \omega}{d \eta_2}$. Therefore, the output is relative degree $\gamma$ if and only if this term is nonzero. 
%     \qed
% \end{proof}
% \vspace{2mm}
% % \begin{remark}
%     In the case $\nn = 1$, the output \eqref{eqn:out} has valid relative degree $\gamma = 1$. 
% % \end{remark}
% Importantly, if $y$ is valid relative degree, each $y^{(i)}$, for $i = 0, \hdots, \gamma -1$ are linearly independent, and form a basis for $\gamma$ dimensions of $\mathcal{X}$ \cite{isidori_elementary_1995}. Defining the error coordinates $\b e$ as in \eqref{eq:error}, we can construct the associated zeroing manifold of the output $y = \eta_1 - \psi_1(\b z)$.
% \begin{lemma} \label{lem:output_zeroing}
% Consider a controlled invariant manifold $\mathcal{M}_{\b\psi}$ and its associated output \eqref{eqn:out}. If the output has relative degree, then $\mathcal{M}_{\b\psi}$ is the zeroing manifold associated \eqref{eqn:out}.
% \end{lemma}
% \begin{proof}
% Valid relative degree implies the existence of unique zeroing manifold $\mathcal{M}_{\b \psi}$, an $\nz$ dimensional surface on which $\b e \equiv 0$ \cite{isidori_elementary_1995}. Because $\mathcal{M}_{\b \psi}$ is controlled invariant and has $y \equiv 0$ (implying derivatives of $y$ are zero), it is also an $\nz$ dimensional zeroing surface; by uniqueness, $\mathcal{M} = \mathcal{M}_{\b \psi}$.
% \qed
% \end{proof}
% \vspace{2mm}
% We have shown that if we construct a mapping $\b \psi$ whose zeroing manifold is controlled invariant, it corresponds with the zeroing manifold of the output \eqref{eqn:out} under the property of valid relative degree.
% If a function $\b \psi$ can be found such that the zero dynamics on $\mathcal{M}_{\b \psi}$ are also stable, then the system can be constructively  stabilized as follows:
% \begin{theorem} \label{thm:zdp_comp_lyap}
%     Consider a relative degree $\gamma$ output  $y = \eta_1 - \psi_1(\b z)$ with zeroing manifold $\mathcal{M}_{\b \psi}$. If the zero dynamics of $\mathcal{M}_{\b \psi}$ are exponentially stable, then any output stabilizing controller $\b k \in \mathcal{K}$ renders the full state $\b x$ exponentially stable.
% \end{theorem}
% \begin{proof}
%     By Lemma \ref{lem:zdp_invariance}, the relative degree of $y$ implies that holding $\b e = 0$ renders $\mathcal{M}_{\b \psi}$ invariant. Since $\mathcal{M}_{\b \psi}$ has exponentially stable dynamics when rendered invariant converse Lyapunov guarantees the existence of $V_{\b z}(\b z)$ satisfying:
%     \begin{align*}
%         k_{1,z} \|\b z\|^2 \leq V_{\b z}(\b z) &\leq k_{2,z} \|\b z\|^2 \\
%         \dot{V}_{\b z}(\b z) = \frac{dV_{\b z}}{d \b z} \b \omega(\b \psi(\b z), \b z) &\leq -k_{3,z} \|\b z\|^2 \\
%         \left\| \frac{dV_{\b z}}{d\b z} \right\| &\leq k_{4,z} \|\b z\|
%     \end{align*}
%     for $k_{i, z}>0$. Applying any controller $k(\b x) \in \mathcal{K}$ (nonempty by virtue of valid relative degree) implies by converse Lyapunov the existence of a Lyapunov function on the error. Define $V_{\b e}(\b e)$ satisfying:
%     \begin{align*}
%         k_{1,e} \|\b e\|^2 \leq V_{\b e}(\b e) &\leq k_{2,e} \|\b e\|^2 \\
%         \dot{V}_{\b e}(\b e) &\leq -k_{3,e} \|\b e\|^2
%         % \left\| \frac{dV_{\b e}}{d\b e} \right\| &\leq k_{4,e} \|\b e\|^2
%     \end{align*}
%     for $k_{i, e} > 0$. We then use the implicit function theorem to establish that $\b \eta$ can be written as a function of $\b e, \b z$:
%     \begin{align*}
%         \b \xi(\b e, \b \eta, \b z) = \b e - \begin{bmatrix}
%         y & \dot{y} & \hdots & y^{(\gamma-1)}
%     \end{bmatrix}^\top = \b 0
%     \end{align*}
%     Observe from \eqref{eqn:output_dot} that $\frac{d\b \xi}{d \b \eta}$ is lower triangular. Furthermore, $(\frac{d\b \xi}{d \b \eta})_{1,1} = 1$ and $(\frac{d\b \xi}{d \b \eta})_{i,i} = (1 - \frac{d\psi_1}{d\b z} \frac{d\b \omega}{d \eta_2})$ for $i=2,\ldots,\gamma$.
%     % , we have:
%     % \begin{align*}
%     %     \frac{d\b \xi}{d \b \eta} = \begin{bmatrix}
%     %         1 & 0 & \hdots & 0 \\
%     %         * & 1 - \frac{d\psi_1}{d\b z} \frac{d\b \omega}{d \eta_2} & \hdots & 0 \\
%     %         \vdots & \vdots & \ddots & \vdots \\
%     %         * & * & \hdots & 1 - \frac{d\psi_1}{d\b z} \frac{d\b \omega}{d \eta_2}
%     %     \end{bmatrix}
%     % \end{align*}
%     % This matrix is invertible since it is lower triangular, and its diagonal elements are nonzero. 
%     By assumption of relative degree, the diagonal elements are nonzero and therefore $\frac{d\b \xi}{d \b \eta}$ is invertible.
%     Therefore, there exists a function $\b \Gamma: \mathcal{E} \times Z \to N$ such that $\b \xi(\b e, \b \Gamma(\b e, \b z), \b z) = 0$. We can then redefine the $\b z$ dynamics in terms of $\b e$ via:% instead of $\b\eta$:
%     \begin{equation*}
%         \Tilde{\b \omega}(\b e, \b z) = \b \omega\left(\b \Gamma(\b e, \b z), \b z\right) = \b \omega(\b \eta, \b z).
%     \end{equation*}
%     Finally, consider the positive definite function $V(\b e, \b z) = \sigma V_{\b e}(\b e) + V_{\b z}(\b z)$, for $\sigma > 0$, whose time derivative is:
%     \begin{align}
%         \dot{V}(\b e, \b z) &= \sigma \dot{V}_{\b e}(\b e) + \frac{dV_{\b z}}{d\b z}\Tilde{\b \omega}(\b e, \b z) \nonumber \\
%         &= \dot{V}_{\b e}(\b e) + \frac{dV_{\b z}}{d\b z}\Tilde{\b \omega}(\b 0, \b z) +\frac{dV_{\b z}}{d\b z}\left(\Tilde{\b \omega}(\b e, \b z) - \Tilde{\b \omega}(\b 0, \b z)\right)\nonumber \\
%         % &\leq -\sigma k_{3,e} \|\b e\|^2 - k_{3,z} \|\b z\|^2 + \left\| \frac{dV_{\b z}}{d\b z}\right\|\| \Tilde{\b \omega}(\b e, \b z) - \Tilde{\b \omega}(\b 0, \b z)\| \\
%         &\leq  -\sigma k_{3,e} \|\b e\|^2 - k_{3,z} \|\b z\|^2 + k_{4,z} L_\omega \|\b e\|\|\b z\| \nonumber\\
%         &= -\begin{bmatrix}
%             \|\b e\| \\ \|\b z\|
%         \end{bmatrix}^\top \begin{bmatrix}
%             \sigma k_{3,e} & -\frac{k_{4,z} L_\omega}{2} \\ -\frac{k_{4,z} L_\omega}{2} & k_{3,z}
%         \end{bmatrix}\begin{bmatrix}
%             \|\b e\| \\ \|\b z\|
%         \end{bmatrix} \label{eqn:quad_form}
%     \end{align}
%     where $L_\omega$ is a Lipshitz constant of $\Tilde{\b \omega}$. Choosing $\sigma > \frac{k_{4,z}^2 L_\omega^2}{4k_{3,e} k_{3,z}}$ renders the matrix positive definite, and the quadratic form \eqref{eqn:quad_form} can be bounded, for $\lambda > 0$:
%     \begin{equation*}
%         \dot{V}(\b e, \b z) \leq -\lambda V(\b e, \b z)
%     \end{equation*}
%     since $V$ can be bounded by quadratic functions, certifying that the $V$ is a Lyapunov function by \eqref{eqn:lyap}. Thus, the composite system is exponentially stable under any controller which exponentially stabilizes the outputs. 
%     \qed
% \end{proof}

% \subsection{Local Existence of Stabilizing Zero Dynamics Policies}
% Around the origin, we demonstrate via construction that $\b \psi$ exists for any locally controllable nonlinear system. 
% To achieve this, we identify a stable zeroing manifold for the linear system and leverage the relationship between a nonlinear system and its linearization to generate an output with stable zero dynamics. 
% % leverage the relationship between a nonlinear system and its linearization to generate an output for the nonlinear system with stable zero dynamics.
% % We will then show that this constitutes a proof of existence for the nonlinear system.
% %
% To this end, consider the linearization of \eqref{eqn:pre_feedback} about the origin:
% \begin{align}
%     % \begin{bmatrix}
%     %     \dot{\eta}_1 \\ \dot{\b \eta}_{2:\gamma-1} \\ \dot{\eta}_{\gamma} \\ \dot{\b z}
%     % \end{bmatrix} &= \begin{bmatrix}
%     %         0 & 1 & \b 0 & \b 0 \\ 0 & 0 & \b I & \b 0 \\ 0 & 0 & \b 0 & \b 0 \\ \frac{\partial \b \omega}{\partial \eta_1} & \frac{\partial \b \omega}{\partial \eta_2} & \frac{\partial \b \omega}{\partial \b \eta_{3:\gamma}} & \frac{d \b \omega}{d \b z}
%     % \end{bmatrix} \begin{bmatrix}
%     %     {\eta_1} \\ {\eta_2} \\ {\b \eta}_{3:\gamma} \\ {\b z}
%     % \end{bmatrix} + \begin{bmatrix}
%     %         0 \\ \b 0 \\ 1 \\ \b 0
%     % \end{bmatrix} u \nonumber \\
%     % &= \begin{bmatrix}
%     %         0 & 1 & \b 0 & \b 0 \\ \b 0 & \b 0 & \b I & \b 0 \\ 0 & 0 & \b 0 & \b 0 \\ \b A_{\eta_1} & \b A _{\b \eta_2} & \b 0 & \b A_{\b z}
%     % \end{bmatrix} \begin{bmatrix}
%     %     {\eta_1} \\ {\eta_2} \\ {\b \eta}_{3:\gamma} \\ {\b z}
%     % \end{bmatrix} + \begin{bmatrix}
%     %         0 \\ \b 0 \\ 1 \\ \b 0
%     % \end{bmatrix} u \nonumber \\
%     % &= \b A \begin{bmatrix}
%     %     \b \eta \\ \b z
%     % \end{bmatrix} + \b B u \label{eq:zd_linearized}
%     \begin{bmatrix}
%         \dot{\eta}_1 \\ \dot{\b \eta}_{2:\gamma-1} \\ \dot{\eta}_{\gamma} \\ \dot{\b z}
%     \end{bmatrix} &= \underbrace{\begin{bmatrix}
%             0 & 1 & \b 0 & \b 0 \\ \b 0 & \b 0 & \b I & \b 0 \\ 0 & 0 & \b 0 & \b 0 \\ \b a_{\eta_1} & \b a_{\eta_2} & \b 0 & \b A_{\b z}
%     \end{bmatrix}}_{\triangleq \b A} \begin{bmatrix}
%         {\eta_1} \\ {\eta_2} \\ {\b \eta}_{3:\gamma} \\ {\b z}
%     \end{bmatrix} + \underbrace{\begin{bmatrix}
%             0 \\ \b 0 \\ 1 \\ \b 0
%     \end{bmatrix}}_{\triangleq \b B} u \label{eq:zd_linearized}
% \end{align}
% with $\b a_{\eta_i} = \frac{\partial \b\omega}{\partial \eta_i}\in \R^{\nz}$ and $ \b A_{\b z} = \frac{d \b \omega}{d \b z} \in \R^{\nz \times \nz}$. First, we identify a manifold invariant under a stabilizing controller:
% \begin{lemma} \label{lem:invsub_lin}
%     % Consider a controller $u = \b K\b x$ which stabilizes \eqref{eq:zd_linearized} such that $\b A-\b B\b K$ has distinct real eigenvalues. 
%     % Then, there exists an $\nz$ dimensional invariant subspace $\mathcal{S}$ which is representable as the level set of a 
%     % , such that for each $\b z$ there exists a unique $\b \eta$ such that $(\b \eta, \b z) \in \mathcal{S}$. 
%     There exists a nonempty set of controllers which stabilize \eqref{eq:zd_linearized} and induce an $\nz$ dimensional invariant subspace $\mathcal{S}$ such that for each $\b z$ there exists a unique $\b \eta$ such that $(\b \eta, \b z) \in \mathcal{S}$.
%     % stabilizing , which under closed-loop control induce an $\nz$ dimensional invariant subspace $\mathcal{S}$
% \end{lemma}
% \begin{proof}
%     By assumption the nonlinear system is locally controllable; therefore\eqref{eq:zd_linearized} is controllable \cite{isidori_elementary_1995}. As such, the system can be stabilized by pole placement. Let $u = -\b K \b x$ be any controller which places the poles at unique locations on the negative real axis. Then the closed loop system, $\b A - \b B\b K$, will have $n$ unique, linearly independent eigenspaces \cite{murray_feedback_systems}. It is therefore possible to pick $\nz$ distinct eigenvectors such that the projection onto $Z$ spans the $Z$ subspace. Let $\b v_1, \hdots, \b v_{\nz} \in \R^{n}$ be these eigenvectors. Define
%     \begin{equation*}
%         \b S = \begin{bmatrix}
%         \b v_1 & \hdots & \b v_{\nz}
%     \end{bmatrix}
%     \end{equation*}
%     Then $\mathcal{S} = \text{span}(\b S)$ is an invariant subspace of the closed loop dynamics, since it is the span of eigenspaces. 
%     % Furthermore, this subspace can be parameterized by $\b z$.
%     Given a point $\b z$, the corresponding point on $\mathcal{S}$ is given by 
%     $$\begin{bmatrix}
%         \b \eta \\ \b z
%     \end{bmatrix} = \b S \left( \begin{bmatrix}
%         0 & I
%     \end{bmatrix} \b S\right)^{-1}\b z = \begin{bmatrix}
%         \b S_{\b \eta}^\top \\ \b I
%     \end{bmatrix}\b z$$
%     where $\b S_{\b \eta} = \begin{bmatrix}
%         \b s_{\eta_1} & \hdots & \b s_{\eta_\gamma}
%     \end{bmatrix}$, with $\b s_{\eta_i} \in \R^{\nz}$. The matrix inverse is well defined since $\b S$ is selected such that its projection onto $\b z$ coordinates spans $Z$. 
%     \qed
% \end{proof}
% \begin{remark}
%     While Lemma \ref{lem:invsub_lin} is proven for a specific form of controller (pole placement), nearly all stabilizing controllers will have $\nz$ dimensional invariant subspaces which are parameterizable by $\b z$.
%     Any such subspace can be chosen, and the resulting $\b S$ can be used in the following analysis. 
% \end{remark}

% \cref{lem:invsub_lin} defines an invariant manifold for the controlled linear system. In order to appeal to composite stability, there must exist a controller rendering $\mathcal{S}$ attractive. This can be achieved by constructing an associated output with valid relative degree. 
% However, from \cite{isidori_elementary_1995}, we know that there may exist zeroing manifolds that do not have valid relative degree. We now show that under the assumption of controllability, $\mathcal{S}$ is the zeroing manifold of a suitable output:

% % We now aim to construct an output whose zeroing manifold is exactly . 
% % Not only does this subspace need to exist, but we need to be able to derive to it.


% \begin{lemma} \label{lem:reldeg_lin}
%     Consider a $\nz$ dimensional subspace $\mathcal{S}$ satisfying \cref{lem:invsub_lin}. The output $y = \eta_1 -\b s_{\eta_1}^\top \b z$ has valid relative degree $\gamma$ and $\mathcal{S}$ is the zeroing manifold for this output. 
% \end{lemma}
% \begin{proof}
%     Take $\b C \triangleq \begin{bmatrix}
%         1 & \b 0 & -\b s_{\eta_1}^\top
%     \end{bmatrix}$ such that $y = \b C \b x$. Consider the closed loop matrix $\b A_{cl} = \b A - \b B \b K$. For compactness, define:
%     \begin{align*}
%         m_k &= -\b s_{\eta_1}^\top \b A_{\b z}^k \b a_{\eta_1}\\
%         q_k &= -\b s_{\eta_1}^\top \b A_{\b z}^k \b a_{\eta_1} - \b s_{\eta_1}^\top \b A_{\b z}^{k+1} \b a_{\eta_2}\\
%         \b O_k &= - \b s_{\eta_1}^\top \b A_{\b z} ^k \\
%         p &= 1 - \b s_{\eta_1}^\top \b a_{\eta_2} 
%     \end{align*}
%     Using these we construct the matrix $\b E \in \R^{\gamma \times n}$:
%     \begin{align}\label{eqn:linE}
%     \setlength\arraycolsep{1.8pt}
%         \b E = \begin{bmatrix}
%             \b C \\ \b C \b A_{cl} \\ \b C\b A_{cl}^2 \\ \vdots \\ \b C \b A_{cl}^{\gamma - 1}
%         \end{bmatrix} = \begin{bmatrix}
%             1 & 0 & 0 & \cdots & 0 & \b O_0 \\
%             m_0 & p & 0 & \cdots & 0 & \b O_1 \\
%             m_1 & q_0 & p & \cdots & 0 & \b O_2 \\
%             \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
%             m_{\gamma - 2} & q_{\gamma - 3} & q_{\gamma - 4} & \cdots & p & \b O_{\gamma - 1}
%         \end{bmatrix}
%     \end{align}
%     Observe that for $i < \gamma - 1$, $\b C \b A_{cl} ^i \b B = 0$, as the $E_{j,\gamma} = 0$ for $j = 1, \ldots, \gamma - 1$. Thus, the output $y$ cannot be of relative degree less than $\gamma$. Assume for contradiction that the output is not relative degree $\gamma$. This implies: 
%     \begin{equation}\label{eqn:contradiction}
%         L_{\b B} L_{\b A_{cl}\b x}^{\gamma - 1} y = \b C\b A_{cl}^{\gamma-1} \b B = p = 1 - \b s_{\eta_1}^\top \b a_{\eta_2} = 0.
%     \end{equation}
%     By \cref{lem:invsub_lin}, $\mathcal{S}$ is $\b A_{cl}$ invariant - this implies the existence of $\b J \in \R^{\nz \times \nz}$ such that $\b A_{cl} \b S = \b S \b J$, i.e. the image of $\b S$ under $\b A_{cl}$ is contained in $\b S$. As $\b C \b S = \b 0$, and $\b C \b A_{cl}^k \b S = \b C \b S \b J^k = 0$ we have that $\b S \in \text{null}(\b E)$. Furthermore, by \eqref{eqn:contradiction} we have $\b C \b A_{cl}^{\gamma - 1} \b B = 0$, and $\b B \in \text{null}(\b E)$. Finally, note that $\b B \notin \b S$, as $\b S$ contains an identity block in the lower $\nz$ rows, while $\b B$ has a corresponding $\b 0$ block. This implies $\text{dim}(\text{null}(\b E)) \geq \text{dim}(\text{span}(\b S, \b B)) = \nz + 1$.
%     % \begin{align*}
%     %     \text{dim}(\text{null}(\b E)) \geq \text{dim}(\text{span}(\b S, \b B)) = \nz + 1.
%     % \end{align*}
%     By Rank Theorem, $\text{rank}(E) + \text{dim}(\text{null}(\b E)) = n$, and therefore,
%     \begin{align*}
%         \text{rank}(\b E) \leq n - (\nz + 1) = \gamma - 1.
%     \end{align*}
%     Therefore, $\b E$ is rank deficient, since it has $\gamma$ rows. There is a nontrivial left nullspace; there exists $\b v = [\alpha_0 \ \hdots \ \alpha_{\gamma - 1}]^\top$, such that $\b v^\top \b E = \b 0$. Without loss of generality\footnote{$\b v$ must have at least one nonzero term since the null space is nontrivial. If $\alpha_{\gamma - 1} = 0$, this proof can be continued by redefining $\b E$ to omit the last row (or as many as necessary such that the last element of $\b v$ is nonzero). Then $\b v$ can be scaled such that its last entry has magnitude 1.}, we take $\alpha_{\gamma-1} = 1$. As the rightmost block of $\b v^\top \b E = \b 0$, 
%    \begin{align}
%        \b O_{\gamma - 1} &= -\sum_{i=0}^{\gamma - 2} \alpha_{i} \b O_i \label{eqn:crit}
%    \end{align}    
%     Next, because $p=0$ by \eqref{eqn:contradiction}, $\b v^\top \b E_{\gamma - 2} = \alpha_{\gamma -1} q_0 = 0$, where $\b E_{i}$ is the $i$'th column of $\b E$. Therefore, $q_0 = 0$. Applying this logic on rows of $\b E$ backward to $\b E_2$ gives:
%     \begin{align*}
%         q_{i} &= 0 \quad \forall i \in \{ 0, \hdots, \gamma - 3\}.
%     \end{align*}
%     Finally, we demonstrate via induction that $q_j = 0$, for any $j \in \mathbb{Z}_+$. Assuming that $q_j = 0$, we aim to show that $q_{j+1} =-\b s_{\eta_1}^\top \b A_{\b z}^{j+1}\left( \b a_{\eta_1} - \b A_{\b z} \b a_{\eta_2}\right)= 0$. Introduce $q_{j+1}$ by right-multiplying \eqref{eqn:crit} by $\b A_{\b z}^{k}(\b a_{\eta_1} - \b A_{\b z} \b a_{\eta_2})$, for $k = j+1-(\gamma - 1)$:
%     \begin{align*}
%         q_{j+1} &= \b O_{\gamma - 1}\b A_{\b z}^{k}(\b a_{\eta_1} - \b A_{\b z} \b a_{\eta_2}) \\
%         &= -\sum_{i=0}^{\gamma - 2}\alpha_{i} \b s_{\eta_1}^\top \b A_{\b z}^{i + k} \b a_{\eta_1} - \sum_{i=0}^{\gamma - 2}\alpha_{i} \b s_{\eta_1}^\top \b A_{\b z}^{i + k + 1} \b a_{\eta_2}.
%     \end{align*}
%     Note that $q_i$ can be rearranged:
%     \begin{align*}
%         -\b s_{\eta_1}^\top \b A_{\b z}^{i} \b a_{\eta_1} = - \b s_{\eta_1}^\top \b A_{\b z}^{i+1}\b a_{\eta_2}.
%     \end{align*}
%     Substituting this for terms $q_{j-(\gamma - 1)}$ to $q_{j}$ into the right sum:
%     \begin{align*}
%         q_{j+1} &= -\sum_{i=0}^{\gamma - 2}\alpha_{i} \b s_{\eta_1}^\top \b A_{\b z}^{i + k} \b a_{\eta_1} + \sum_{i=0}^{\gamma - 2}\alpha_{i} \b s_{\eta_1}^\top \b A_{\b z}^{i + k } \b a_{\eta_1} = 0.
%     \end{align*}
%     And the inductive step has been shown. The base case holds trivially for $\gamma \geq 3$ by the structure of $\b E$, and $\b C \b B = 1$ for relative degree one systems (trivially valid relative degree). It remains to show the base case holds for $\gamma = 2$.  

%     First, examine the fact that $\mathcal{S}$ is invariant under $\b A_{cl}$.
%     Expanding $\b A_{\text{cl}} \b S = \b S \b J$, given that $\b K = [k_{\eta_1} \ k_{\eta_2} \ \b k_{\b z}]$:
%     \begin{align*}
%         \begin{bmatrix}
%                 \b s_{\eta_2}^\top \\-k_{\eta_1} \b s_{\eta_1}^\top - k_{\eta_2} \b s_{\eta_2}^\top - \b k_{\b z}
%              \\ \b a_{\eta_1} \b s_{\eta_1}^\top + \b a_{\eta_2} \b s_{\eta_2}^\top + \b A_{\b z}
%         \end{bmatrix} &= \begin{bmatrix}
%                 \b s_{\eta_1}^\top\b J \\ \b s_{\eta_2}^\top\b J \\ \b J
%         \end{bmatrix}
%     \end{align*}
%     Right multiply the second equation by $\b a_{\eta_2}$, and using \eqref{eqn:contradiction}:
%     \begin{align*}
%         \b a_{\eta_1} + \b A_{\b z} \b a_{\eta_2} = (\b I - \b a_{\eta_2}\b s_{\eta_1} ) \b J \b a_{\eta_2}
%     \end{align*}
%     And note that left multiplying by $\b s_{\eta_1}$ gives:
%     \begin{align*}
%         q_0 = \b s_{\eta_1}^\top (\b a_{\eta_1} + \b A_{\b z} \b a_{\eta_2}) = \b s_{\eta_1}^\top(\b I - \b a_{\eta_2}\b s_{\eta_1}^\top ) \b J \b a_{\eta_2} = 0
%     \end{align*}
%     again leveraging $\b s_{\eta_1}^\top \b a_{\eta_2} = 1$. We have established the based case for induction, for relative degree $\gamma = 2$. 

%     We now aim to demonstrate the contradiction, by showing that \eqref{eqn:contradiction} leads to the system losing controllability.
%     Consider the controllability matrix of the system. Controllability is preserved under feedback, so we examine $\mathscr{C}(\b A, \b B)$: 
%     \begin{align*}
%         \mathscr{C}(\b A, \b B) &= \begin{bmatrix}
%             \b 0  & 1 & 0 & \hdots & 0\\
%             \b I  & 0 & 0 & \hdots & 0\\
%             \b 0 & \b a_{\eta_2} & \b Q_0 & \hdots & \b Q_{n-(\gamma + 1)}
%         \end{bmatrix} \\
%         \b Q_i &= \b A_{\b z}^{i}(\b a_{\eta_1} + \b A_{\b z} \b a_{\eta_2})
%     \end{align*}
%     We finish by showing the $\b C$ is in the left null space of $\mathscr{C}$:
%     \begin{align*}
%         \b C \mathscr{C} = \begin{bmatrix}
%             0 & p & q_0 & \hdots & q_{n-(\gamma + 1)}
%         \end{bmatrix} = \b 0
%     \end{align*}
%     And therefore $\mathscr{C}$ is not full rank. We have reached contradiction, and $y$ must be relative degree $\gamma$. 
%     Finally, note that $\mathcal{S}$ is the zeroing surface associated with $y$ by \cref{lem:output_zeroing}.
%     \qed
% \end{proof}
% \cref{lem:reldeg_lin} constructs an output and its associated zeroing manifold such that 1) the output has valid relative degree, and 2), the zeroing manifold is exponentially stable. Now, we show that the output locally retains both of these properties under the nonlinear dynamics:
% \begin{theorem} \label{thm:local_existance}
%    \textit{Given a system \eqref{eqn:pre_feedback}, the output $y = \eta_1 - \b s_{\eta_1}^\top\b z$ obtained in \cref{lem:reldeg_lin} has valid relative degree, and its zero dynamics are exponentially stable for the nonlinear system. As such, stabilizing $\b e \rightarrow 0$ results in stability of the entire system in a neighborhood of the origin.}
% \end{theorem}

% It is important to emphasize that \cref{thm:local_existance} gives a completely \emph{constructive method for stabilizing a broad class of underactuated systems using output stabilization}. In the results section, we demonstrate this constructive method on a canonical example of underactuation, the cartpole.


% \vspace{0.2cm}
% \begin{proof}
%     First, we establish that the output is relative degree $\gamma$ for the nonlinear system. The output has the form $y = \b C \b x = \eta_1 - \b s_{\eta_1}^\top \b z$. By \cref{lem:zdp_invariance}, we have that $L_{\b g}L_{\b f}^jy(\b x) \equiv 0$ for $j = 0,\ldots, \gamma-2$ and:
%     \begin{align*}
%         L_{{\b g}} L_{{\b f}}^{\gamma - 1} y &= 1 - \b s_{\eta_1}^\top \frac{d \b \omega}{d \eta_2}.
%     \end{align*}
%     For relative degree, we need $L_{{\b g}} L_{{\b f}}^{\gamma - 1} y \neq 0$. 
%     \begin{align*}
%         L_{{\b g}} L_{{\b f}}^{\gamma - 1} y &= 1 - \b s_{\eta_1}^\top \frac{d \b \omega}{d \eta_2}\\
%         &= \underbrace{1 - \b s_{\eta_1}^\top \b a_{\eta_2}}_{\b C \b A^{\gamma - 1} \b B} + \underbrace{\b s_{\eta_1}^\top \left(\b a_{\eta_2} - \frac{d \b \omega}{d \eta_2} \right)}_{\triangleq \Delta(\b x)}
%     \end{align*}
%     where $\Delta: \mathcal{X} \to \R$. \cref{lem:reldeg_lin} assures that $|\b C\b A^{\gamma - 1} \b B| = \delta > 0$. To guarantee $L_{{\b g}} L_{{\b f}}^{\gamma - 1} y \neq 0$, we bound $|\Delta(\b x)| < \delta$. 
%     \begin{align*}
%         \left| \Delta(\b x) \right| &\leq \|\b s_{\eta_1}\| \left\|\b a_{\eta_2} - \frac{d\b \omega}{d \eta_2}\right\|
%     \end{align*}
%     Note that the function $\left\|\b a_{\eta_2} - \frac{d\b \omega}{d \eta_2}\right\|$ is continuous and zero at the origin. Therefore, there exists an $\varepsilon > 0$ such that
%     \begin{align*}
%         \left\|\b a_{\eta_2} - \frac{d\b \omega}{d \eta_2}\right\| \leq \frac{\delta}{2 \|\b s_{\eta_1}\|} \quad \forall \ (\b \eta, \b z) \in B_\varepsilon(\b 0, \b 0)
%     \end{align*}
%     Inside this epsilon ball, we have $|\Delta(\b x)| \leq \frac{1}{2}\delta$, and therefore $|L_{{\b g}}L_{{\b f}}^{\gamma - 1}y | > \frac{1}{2}\delta$. Locally, the output has valid relative degree for the nonlinear system. 

%     It remains to show that the zeroing manifold, $\mathcal{M}_{\b \psi}$ of this output is stable for the nonlinear system. First, given the error coordinates \eqref{eq:error}, consider $\frac{d \b e}{d \b x} = \begin{bmatrix}
%         \frac{d\b e}{d \b \eta} & \frac{d \b e}{d \b z}
%     \end{bmatrix}$ evaluated at the origin. For a row of this matrix,
%     \begin{align}
%         \frac{d}{d \b x}\b e_i \bigg\vert_{\b x = \b 0} &= \frac{d}{d\b x} L_{\b f}^i y\bigg\vert_{\b x = \b 0} \nonumber \\
%         &= \frac{d^2 L_{\b f}^{(i-1)} y}{d\b x^2}\b f\bigg\vert_{\b x = \b 0} + \frac{d}{d\b x}L_{\b f}^{(i-1)} y\frac{d \b f}{d\b x}\bigg\vert_{\b x = \b 0}  \nonumber \\
%         &= \frac{d}{d\b x}L_{\b f}^{(i-1)} y\frac{d \b f}{d\b x}\bigg\vert_{\b x = \b 0} \label{eqn:e_induct}\\
%         &= \b C \b A^i \nonumber
%     \end{align}
%     where the third lines holds by $\b f(\b 0) = \b 0$ and the last equality can be shown by induction. The base case holds as $\frac{dy}{d\b x} = \b C$, and the induction step is given by \eqref{eqn:e_induct}. We have:
%     \begin{align}
%         \frac{d \b e}{d \b x}\bigg\vert_{\b x = \b 0} = \begin{bmatrix}
%             \b C \\ \vdots \\ \b C \b A^{\gamma - 1}
%         \end{bmatrix}
%     \end{align}
%     which is precisely the same as \eqref{eqn:linE}. Therefore, $\frac{d \b e}{d \b \eta}$ is lower triangular with nonzero elements on the diagonal, and is thus invertible. By the implicit function theorem, there exists $\b \psi: Z \to N$ such that $\b e(\b \psi(\b z), \b z) = \b 0$. We aim to show that $\mathcal{M}_{\b \psi}$ is stable. Consider that by the implicit function theorem:
%     \begin{align}
%         \frac{d \b \psi}{d \b z} = -\frac{d \b e}{d \b \eta}^{-1} \frac{d \b e}{d \b z}. \label{eq:dpsi_dz}
%     \end{align}
%     Furthermore, note that since $\frac{d\b e}{d \b x}\vert_{\b x = \b 0} = \b E$, \eqref{eq:dpsi_dz} also holds for the linearization. 
%     % But for the linearization, $\b \psi_{lin}(\b z) = \b S_{\b \eta} \b z$, and thus $\frac{d \b \psi_{lin}}{d \b z} = \b S_{\b \eta}$. 
%     Therefore, at the origin, the tangent space of $\mathcal{M}_{\b \psi}$ for the nonlinear system is equal to the invariant subspace used by the linearization to design the output, i.e. $\frac{d\b e}{d \b \eta}\vert_{\b x = \b 0} = \b S_{\b \eta}$. On $\mathcal{M}_{\b \psi}$ we have $\b \eta = \b \psi(\b z)$, or equivalently:
%     \begin{align*}
%         \b \eta &= \frac{d\b \psi}{d\b z}\bigg\vert_{\b x = \b 0}\b z + \left(\b \psi(\b z) - \frac{d\b \psi}{d\b z}\bigg\vert_{\b x = \b 0}\b z\right) \\
%         &= \b S_{\b \eta}\b z + \underbrace{\left(\b \psi(\b z) - \b S_{\b \eta}\b z\right)}_{\Gamma(\b z)}
%     \end{align*}
%     By mean value theorem, there exists $\varepsilon > 0$ such that inside a ball $B_\varepsilon(\b 0, \b 0)$ we have 
%     \begin{equation*}
%         \|\Gamma(\b z)\| \leq N_\Gamma(\varepsilon) \|\b z\|
%     \end{equation*}
%     With $N_\Gamma(\varepsilon) \rightarrow 0$ as $\varepsilon \rightarrow 0$. 

%     Finally, given that the surface $\mathcal{S}$ is stable under the linearized dynamics from Lemma \ref{lem:invsub_lin}, converse Lyapunov guarantees the existence of a function $V_{\b z}(\b z)$ satisfying
%     \begin{align*}
%         k_1 \|\b z\|^2 \leq V_{\b z}(\b z) &\leq k_2\|\b z\|^2 \\
%         \dot{V}_{\b z}(\b z) &= \frac{dV_{\b z}}{d\b z}\left(\b a_{\eta_1} \b s_{\eta_1} + \b a_{\eta_2} \b s_{\eta_2} + \b A_{\b z}\right)\b z \\&\leq -k_3 \|\b z\|^2 \\
%         \left\|\frac{dV_{\b z}}{d\b z}\right\| &\leq k_4 \|\b z\|
%     \end{align*}
%     for $k_i > 0$. We aim to show that this function is also a Lyapunov function for the dynamics on the nonlinear zeroing manifold, where $(\b \eta, \b z) = (\b \psi(\b z), \b z)$. To this end, define $\Tilde{\b A} \in \R^{\nz \times \nz}$ and $\b \Delta_1, \b \Delta_2: Z \to \R^{\nz}$: 
%     \begin{align*}
%         \Tilde{\b A} &= \b a_{\eta_1} \b s_{\eta_1} + \b a_{\eta_2} \b s_{\eta_2} + \b A_{\b z} \\
%         \b \Delta_1(\b z) &= \b \omega\left(\b S_{\b \eta} \b z, \b z\right) - \Tilde{\b A}\b z \\
%         \b \Delta_2(\b z) &= \b \omega\left(\b \psi(\b z), \b z\right) - \b \omega\left(\b S_{\b \eta}, \b z\right)
%     \end{align*}
%     Differentiate $V_{\b z}$ under the nonlinear dynamics:
%     \begin{align*}
%         \dot{V}_{\b z} &= \frac{dV_{\b z}}{d\b z}\b \omega\left(\b \psi(\b z), \b z\right) \\
%         &=\frac{dV_{\b z}}{d\b z}\Tilde{\b A}\b z + \frac{dV_{\b z}}{d\b z}\left(\b \Delta_1(\b z) + \b \Delta_2(\b z) \right)        
%     \end{align*}
%     Noting that $\b \Delta_1(\b z)$ is the error in the linearization of $\b \omega$ on the linear surface $\mathcal{S}$, it can be bounded using mean value theorem as $\|\b \Delta_1(\b z)\| \leq N_1(\varepsilon) \|\b z\|$. Similarly, $\b \Delta_2$ can be bounded using Lipschitz continuity of $\b \omega$, and the fact that $\b \psi(\b z) - \b S_{\b \eta}\b z = \b \Gamma(\b z)$ to obtain $\|\b \Delta_2(\b z)\| \leq L_{\b \omega} N_\Gamma(\varepsilon) \|\b z\| = N_2(\varepsilon)\|\b z\|$. Letting $N = N_1 + N_2$, we have
%     \begin{align*}
%         \left\|\frac{dV_{\b z}}{d\b z}\left(\b \Delta_1(\b z) + \b \Delta_2(\b z) \right)\right\| &\leq \left\|\frac{dV_{\b z}}{d\b z}\right\|\left(\|\b \Delta_1(\b z)\| + \|\b \Delta_2(\b z)\| \right) \\
%         &\leq k_4 N(\varepsilon) \|\b z\|^2
%     \end{align*}
%     Choosing $\varepsilon > 0$ such that $N(\varepsilon) < \frac{k_3}{2k_4}$, we have
%     \begin{align*}
%         \dot{V}_{\b z}(\b z) & \leq -k_3\|\b z\|^2 + k_4 N(\varepsilon)\|\b z\|^2 \\
%         &\leq - \frac{k_2}{2}\|\b z\|^2
%     \end{align*}
%     Therefore, we see that $V_{\b z}$ is a Lyapunov function on the nonlinear zeroing manifold, with a sufficiently small ball around the origin. We have successfully demonstrated that $\b \psi$ has the required properties to apply Theorem \ref{thm:zdp_comp_lyap} and conclude local exponential stability of the composite system. 
%     \qed
% \end{proof}
% \vspace{2mm}

% This proof uses linearization to design an output which has desirable properties. Locally, the zeroing manifold for this output $\mathcal{M}_{\b \psi}$ is close to the linear systems zeroing manifold (captured by $\b \Delta_2$), and the zero dynamics are close to the dynamics of the linear system (captured by $\b \Delta_1$). Sufficiently close to the origin, relative degree and stability of $\mathcal{M}_{\b \psi}$ are retained for the nonlinear system.



% % In order for this manifold to be invariant, we require that $\dot {\b x} \in \textsc{T} _\b x\mathcal{M}$, which can equivalently by written as $$\langle\partial \b e, \dot {\b x}\rangle|_{\b x\in\mathcal{M}} = 0$$ as the gradient field of a function provides a basis for the annihilator of its tangent space. In doing so, we will be able to use output tracking to this manifold to recover stability and bounded suboptimality of the overall system. 

% % Suppose for the moment that such a function $\func$ exists with $\func(\b 0) = \b 0$ -- we will begin by analyzing the properties of this function, and will later provide constructive means of generating it. Invariance of $\mathcal{M}$ under optimal control implies:
% % \begin{align}
% % 	\hat{\b f}(\b \psi(\b z), \b z) + \hat{\b g}(\b \psi(\b z), \b z) \b u^*(\b z) = \frac{d\b\psi}{d\b z} \b\omega(\b \psi(\b z), \b z). \label{eq:inv}
% % \end{align}
% % where $\b u^*$ is the minimizer of \eqref{eq:hjb} at the point $(\func(\b z), \b z)$.

% \section{Optimal Control for Learning Zero Dynamics Policies}

% While the linearization of a system about equilibrium can be used to construct locally stabilizing controllers, it is desirable to obtain larger regions of attraction, and leverage the nonlinear dynamics of the system. Therefore, we aim to construct $\man$ satisfying controlled invariance and stability.

% \subsection{Optimal Control for Stabilization}


% As asymptotic stability is a necessary condition for optimality \cite{liberzon_calculus_2012}, we leverage optimal control to find $\man$. Consider the infinite-time optimal control problem:
% \begin{align}
%     % \b u^*(\b \eta, \b z)
%     V(\b x_0) \triangleq \min_{\substack{\b x,  \b u}}\quad & \int_0^\infty c(\b x(t),  \b u(t)) dt \label{eqn:ocp}\\
% \textrm{s.t.} \quad & \dot {\b x} = {\b f}(\b x) + \b g(\b x) \b u \notag
% \end{align}
% where $V: \mathcal{X} \rightarrow \R$ is the value function and $c:\mathcal{X} \times \mathcal{U} \to \R$ is a positive definite cost function. In order to apply \cref{thm:zdp_comp_lyap}, we will require exponential stability on the manifold. Therefore, we begin by state conditions under which the optimal controller is exponentially stabilizing:
% \begin{theorem}
%     \textit{Let $V(\b x)$ be the value function for the optimal control problem defined \eqref{eqn:ocp}, with quadratic cost $c(\b x, \b u) = \b x^\top \b Q \b x + ru^2$ and compact state space $\mathcal{X}$.  The nonlinear system is exponentially stable under the optimal controller. }
% \end{theorem}
% \begin{proof}
%     In a sufficiently small ball around the origin, the LQR approximation of the optimal controller, obtained by linearizing the dynamics about equilibrium, will be exponentially stabilizing for the nonlinear system \cite{sastry_linearization_1999}, as it locally satisfies input bounds. This implies constants $M_{LQR}, \ \lambda_{LQR}, \ \delta > 0$ such that:
%     \begin{align*}
%     \|\b x_0\| \leq \delta  \quad \implies \quad 
%         \|\b x(t)\| \leq M_{LQR}e^{-\lambda_{LQR} t} \|\b x_0\|
%     \end{align*}
%     We aim to show that the trajectory emanating from an arbitrary initial condition $\b x_0 \in B_\delta(\b 0)$ is exponentially stable. For any $M,\lambda > 0$, consider the set:
%     \begin{align*}
%         T = \{ t \in \R_{\geq 0} ~\vert~ \|\b x(t)\| > Me^{-\lambda t} \|\b x_0\| \}
%     \end{align*}
%     We condition on whether there is an upper bound to the elements of $T$:
    
%     \proofsubstep{Case 1:} There exists an upper bound $\overline{T}$ such that $t < \overline{T}$ for all $t \in T$. Then consider the maximum violation ratio
%     \begin{align*}
%         \overline{r} = \sup_{t \in T} \frac{\|\b x(t)\|}{Me^{-\lambda t} \|\b x_0\|} \leq \frac{B}{Me^{-\lambda \overline{T}}\|\b x_0\|} 
%     \end{align*}
%     Take $\overline{r} = 1$ if $T$ is empty. Then:
%     \begin{align*}
%         \|\b x(t)\| \leq \overline{r}Me^{-\lambda t} \|\b x_0\|
%     \end{align*}
%     implying the trajectory is exponentially stable.
    
%     \proofsubstep{Case 2:} There is no upper bound on the elements in $T$. We will establish $V(\b x)$ is a Lyapunov function certifying exponential stability of the trajectory. Bound the decrease rate:
%     \begin{align}
%         \dot{V}(\b x) &= -\b \left(\b x^\top \b Q \b x + ru^2 \right) \nonumber \\
%         &\leq -\underline{\lambda}(\b Q) \|\b x\|^2 \label{eq:value_dot}
%     \end{align}
%     Next, bound $V$ above by a quadratic function. Because LQR is suboptimal for the nonlinear system, applying it can only increase the cost relative to $V(\b x)$:
%     \begin{align*}
%         V(\b x_0) &\leq \int_0^\infty \b x^\top \b Q \b x + r(\b K \b x)^2 dt \\
%         &\leq \int_0^\infty \b (\overline{\lambda}(\b Q) + r \overline{\lambda}(\b K^\top \b K)) \|\b x\|^2 dt\\
%         &\leq \int_0^\infty \b (\overline{\lambda}(\b Q) + r \overline{\lambda}(\b K^\top \b K)) M_{LQR}^2 e^{-2\lambda t}\|\b x_0\|^2 dt\\
%         &= \frac{(\overline{\lambda}(\b Q) + r \overline{\lambda}(\b K^\top \b K)) M_{LQR}^2}{2\lambda_{LQR}} \|\b x_0\|^2
%     \end{align*}
%     with $\overline{\lambda}, \underline{\lambda}$ the maximum and minimum eigenvalues respectively. Finally, lower bound $V(\b x)$ by a quadratic.
%     \begin{align*}
%         V(\b x_0) &= \int_0^\infty \b x^\top \b Q \b x + ru^2 dt \\
%         &\geq \int_T \underline{\lambda}(\b Q) \|\b x\|^2 dt\\
%         &\geq \underline{\lambda}(\b Q) M^2 \|\b x_0\|^2 \left(\int_T e^{-2\lambda t}  dt \right) \\
%         &= \underline{\lambda}(\b Q) M^2 \|\b x_0\|^2 \left(\int_0^\infty e^{-2\lambda t}  dt - \int_{\R_{\geq 0} \backslash T} e^{-2\lambda t}  dt\right) \\
%         &= \underline{\lambda}(\b Q) M^2\left(\frac{1}{2\lambda} -c \right)\|\b x_0\|^2
%     \end{align*}
%     where $\frac{1}{2\lambda} -c > 0$ as both integrals integrate over the same strictly positive function, but the integral corresponding to $c$ does so over a smaller domain\footnote{To make this precise, one must acknowledge that the set $T$ has nonzero measure (which it must, due to continuity of solutions and the strict inequality used to define it), and utilize Lebesgue integration. }. The above bounds hold at each point on the trajectory, and therefore $V$ is a Lyapunov function certifying exponential stability of the trajectory.

%     As the above argument holds for all $\b x \in B_\delta(\b 0)$, exponential convergence holds over this ball. We how aim to extend this claim over the compact state space $\mathcal{X}$. At $V \succ 0$ and $\dot{V} \prec 0$, we have that the optimal controller is asymptotically stabilizing \cite{liberzon_calculus_2012}. By compactness of $\mathcal{X}$ and \eqref{eq:value_dot}, the time for a trajectory to enter $B_\delta(\b 0)$ is bounded by:
%     \begin{align*}
%         T_{\max} = \frac{\sup_{\b x_0 \in \mathcal{X}} V(\b x_0)}{\inf_{\b x_0 \in \mathcal{X} \backslash B_\delta(\b 0)} \dot{V}(\b x_0)} \leq  \frac{\sup_{\b x_0 \in \mathcal{X}} V(\b x_0)}{\underline{\lambda}(\b Q) \delta^2}
%     \end{align*}
%     Because trajectories in $B_\delta(\b 0)$ converge exponentially:
%     \begin{align*}
%         \|\b x(t)\| \leq Me^{-\lambda (t - T_{\max})} \|\b x_{T_{\max}}\| \quad \forall t > T_{\max}
%     \end{align*}
%     By compactness of $\mathcal{X}$, trajectories are bounded by $\|\b x\| \leq B$, and the whole trajectory can be bounded exponentially:
%     \begin{align*}
%         \|\b x(t)\| \leq \frac{\max\{M, B\} e^{\lambda T_{\max}}}{\min\{1, \delta\}}e^{-\lambda t} \|\b x_0\| 
%     \end{align*}
%     The optimal controller is exponentially stabilizing.
%     \qed
% \end{proof}
% \vspace{2mm}

% \subsection{Learning Zero Dynamics Policies}


% We propose a learning algorithm to find functions $\b \psi$ such that $\mathcal{M}_{\b \psi}$ is controlled invariant, and that the zero dynamics on $\mathcal{M}_{\b \psi}$ are stable. This this end, we search for manifolds which are invariant under optimal control. Let $u^*(\b x)$ be the solution to the optimal control problem \eqref{eqn:ocp}. Then $\mathcal{M}_{\b \psi}$ is invariant under optimal control if 
% \begin{align*}
%     \begin{bmatrix}
%         \b I & -\frac{d \b \psi}{d\b z}
%     \end{bmatrix} \begin{bmatrix}
%         \hat{\b f}(\b \eta, \b z) + \hat{\b g}(\b \eta, \b z) u^*(\b x) \\
%         \b \omega(\b \eta, \b z)
%     \end{bmatrix} = \b 0
% \end{align*}
% Given a neural network parameterization of $\b \psi_{\b \theta}$, we define the loss function
% \begin{align} \label{eqn:loss}
%     L(\b \theta) = \mathbb{E}_{\b z \sim D} \left\|\hat{\b f}(\b \eta, \b z) + \hat{\b g}(\b \eta, \b z) u^*(\b x) - \frac{d \b \psi}{d\b z}\b \omega(\b \eta, \b z) \right\|
% \end{align}
% At zero loss, the manifold is invariant under the optimal controller. This satisfies both of the required properties of $\mathcal{M}_{\b \psi}$; the loss function enforces invariance, and optimality enforces stability. We minimize this loss using stochastic gradient descent.


% % \section{Results and Limitations}

% \subsection{Application to the Cartpole}

% To demonstrate the effectiveness of the zero dynamics policy, we deploy it on the canonical underactuated system, the cartpole. We apply three controllers: 1) LQR from the linearization about equilibrium 2) LQR ZDP, the zero dynamics policy constructed as in \cref{thm:local_existance}, from the LQR controller stabilizing the linearization about equilibrium, and 3) Learned ZDP, where we minimize the loss function \eqref{eqn:loss} under the LQR controller. Despite all three controllers relying on \textit{identical} LQR controllers under the hood, \cref{fig:theory} demonstrates that tracking the LQR ZDP improves the region of attraction over LQR, while learning a nonlinear surface improves the region of attraction even further. 
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/RoA_tmp.jpg}
%     \caption{A section ($x = \dot{x} = 0$) of the region of attraction for various controllers of the destabilized cartpole.}
%     \label{fig:theory}
%     \vspace{-4mm}
% \end{figure}

% It is interesting to highlight intuitive reasons for this progressive improvement, even though all policies are based on the same LQR controller. 
% % First note that \textit{on the zeroing surfaces} all controllers are approximately equal (the learned surfaces may not be exactly invariant under the LQR policy, and will differ slightly). The section shown uses $\dot{\theta}$ rather than the second $\b z$ coordinate, and does not represent the dynamics on the surface, allowing us to see differences between the approaches. 
% The LQR ZDP policy incorporates more nonlinear model information than LQR alone, by feedback linearizing while stabilizing to the manifold defined by the LQR policy. This causes it to behave more aggressively than the LQR controller, and stabilizes over a larger space. Next, the learned ZDP finds a manifold which is not linear; this gives it more flexibility, and extends the validity of the model over a larger region. Finally, stabilizing the manifold with PD control instead of feedback linearization avoids issues with loss of relative degree, where control inputs blow up and integration is unstable for FBL. This allows for an even larger region of attraction (in this case), as the PD controller is still pushing 'in the right direction' even if it isn't matching the exponential rate of convergence demanded by the FBL controller. 

% \section{Conclusion}



% % \clearpage

% % \section{Appendix}
% % \begin{proof}[Proof of Proposition \eqref{prop:bijection}]
% %     Consider $D\b\Phi$, given by:
% %     \begin{equation} 
% % D\Phi(q, \dot{q}, t) = \begin{bmatrix}
% % B^\top & 0 \\ 0 & B^\top \\ N & 0 \\ \frac{\partial}{\partial q} ND(q)\dot{q} & ND(q) \end{bmatrix}
% % \end{equation}
% % This Jacobian is full rank at all points in the state space and in time (this can be seen by rearranging the rows to create and identity element in the top left), and noting that $ND(q) = \begin{bmatrix} D_{11}(q) & D_{12}(q)\end{bmatrix}$ where $D_{11}(q)$ is the upper right $n-m \times n-m$ square block of the inertia matrix and is thus invertible. 
% % \end{proof}

% % \begin{section}{Proofy type things}
% % I see the flow of logic going: 
% % \begin{enumerate}
% %     \item nonlinear system controllable iff linearization is controllable. Now consider the linearization of a nonlinear robotic system in the 'canonical normal form' we have proposed.
% %     \item Prove this linear system has a subspace of proper dimension with stable dynamics, which when stabilized, stabilizes the whole system.
% %     \item Prove that locally, this subspace (a) still has valid relative degree - can be stablized, and (b) still has stable dynamics, and thus defines a ZD surface for the nonlinear system. 
% % \end{enumerate}
% % The above items are quiet general, can be proven without strong assumptions (local controllability, standard robotic system form is the only ones I see). There is another set of statements which we can attempt to make regarding optimal controllers, which is different in flavor. This has the power to be less 'local', but will perhaps require assumptions on the form of the optimal controller. Note that any stabilizing controller can be used, the 'optimal' one is only relevant inasmuch as there are algorithm ways of computing it. 
% % \begin{enumerate}
% %     \item A surface which is invariant under a stabilizing controller is stable. 
% %     \item If the surface can be constructively stabilized (valid relative degree, ect), then there is a constructive method for stabilizing the entire system. Composite Lyapunov.
% %     \item Propose a loss function, which at zero loss, renders a surface which is invariant under optimal curves. Stabilizing this surface stabilizes the entire system. 
% %     \item Show that ultimately bounded loss results in ISS behavior.
% % \end{enumerate}
% % These proofs can be done if the controller is Lipschitz continuous (spatially as well as along trajectories). If the controller is not locally Lipschitz, the flows can have spatial discontinuities, and it becomes difficult to think about 'surfaces' at all, as they may not be manifolds. Note that in general, optimal controllers are not even Lipschitz along trajectories (bang-bang behavior), and if they are, they are not Lipschitz spatially (topological obstructions, ect). Regions along which optimal feedback is Lipschitz becomes important here. 

% % \textcolor{red}{
% % Looking at this outline farther, it may make sense to begin with some statements from the second column. First, outline desired properties - a surface which can be rendered invariant and has stable dynamics, then converse Lyapunov, gives stability of the entire system. Then show that locally, such surfaces always exist for controllable nonlinear underactuated robotic systems. End with optimality/loss function as algorithmic way of finding such functions.} 
% % \end{section}
% \bibliographystyle{ieeetr}
% \balance
% \bibliography{references}

% % % \section{Related Work}

% % \input{Sections/Conclusion.tex}

% % \clearpage
% % \section{Acknowledgements} 
% % The authors would like to thank Murtaza Hathiyari for his assistance with hardware implementation.

% % % Acknowledgments---Will not appear in anonymized version
% % % \acks{We thank a bunch of people.}

% % %
% % \bibliography{Zero Dynamics Policies}

% \end{document}


==> noels_notes.tex <==
% % \documentclass[conference]{IEEEtran}
% \usepackage{times}

% % numbers option provides compact numerical references in the text. 
% \usepackage[numbers]{natbib}
% \usepackage{multicol}
% \usepackage[bookmarks=true]{hyperref}

% % The following packages will be automatically loaded:
% % amsmath, amssymb, natbib, graphicx, url, algorithm2e

% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{graphicx}
% \usepackage{epstopdf}
% \usepackage{mathtools}
% \usepackage{dsfont}
% \usepackage{tikz}
% \usepackage{siunitx}
% \usepackage{hyperref}
% \usepackage[font=footnotesize]{caption}
% % \usepackage{floatrow}
% \usepackage[noabbrev,capitalize]{cleveref}
% \usepackage{balance}    % have even columns on last page
% \usepackage{xcolor}
% \usepackage{tcolorbox}
% % \usepackage{algorithm}
% % \usepackage{algpseudocode}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% % \usepackage{algorithm2e}
% \usepackage{mathtools}
% \usepackage{dsfont}
% \usepackage{mathrsfs}
% % \usepackage[noadjust]{cite} % multiple citations are combined
% \usepackage{stmaryrd}
% \usepackage{placeins}
% \usepackage{upgreek}
% \usepackage{wrapfig}
% \usepackage{bm}
% \usepackage{cases}
% \usepackage{bbm}
% \usepackage{noel}

% % \usepackage[backend=biber, natbib=true, style=apa, hyperref=true, firstinits=true, maxcitenames=1, parentracker=true, maxbibnames=99]{biblatex}
% % \addbibresource{./references.bib}

% \DeclareMathOperator*{\argmin}{argmin}
% \DeclareMathOperator*{\argmax}{argmax}   

% \title{Zero Dynamics Policies}
% % Use \Name{Author Name} to specify the name.
% % If the surname contains spaces, enclose the surname
% % in braces, e.g. \Name{John {Smith Jones}} similarly
% % if the name has a "von" part, e.g \Name{Jane {de Winter}}.
% % If the first letter in the forenames is a diacritic
% % enclose the diacritic in braces, e.g. \Name{{\'E}louise Smith}

% % Two authors with the same address
% % \coltauthor{\Name{Author Name1} \Email{abc@sample.com}\and
% %  \Name{Author Name2} \Email{xyz@sample.com}\\
% %  \addr Address}

% % Three or more authors with the same address:
% % \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
% %  \Name{Author Name2} \Email{an2@sample.com}\\
% %  \Name{Author Name3} \Email{an3@sample.com}\\
% %  \addr Address}

% % Authors with different addresses:


% \begin{document}

% \author{Author Names Omitted for Anonymous Review. Paper-ID [add your ID here]}

% \maketitle


% \vspace{-6mm}
% \begin{abstract}%
% Stabilizing underactuated systems remains a challenging task in control theory due to the existence of fundamental limits on how the control input can effect the system dynamics. The decomposition of such systems into actuated and unactuated states, namely output and zero dynamics coordinates, has provided useful insight into the underlying structure that exists, but has yet to result in constructive ways to stabilize such systems. Despite these fundamental limits, modern control approaches such as Model Predictive Control (MPC) and Reinforcement Learning (RL) have demonstrated a surprising ability to stabilize such systems, but have largely overlooked the underlying structure that is present. The goal of this work is to reconcile these two perspectives by analyzing the way in which MPC and RL are able to stabilize these underactuated states, and in doing so developing a canonical, low-dimensional action space through which learned policies can stabilize the full system state. Specifically, we formalize the idea of zero dynamics policies -- policies which map from the underactuated states of a system to the output space -- and provide conditions under which stabilization of the full system state can be achieved.
% \end{abstract}

% \IEEEpeerreviewmaketitle

% % \begin{keywords}%
% %   bipedal locomotion, zero dynamics, safety, robotics
% % \end{keywords}

% % \blfootnote{$^*$ These authors contributed equally to this work.}
% % \vspace{-4mm}
% % \section{Introduction}
% % % \input{Sections/Introduction}
% % \input{Sections/Introduction_v2}

% \section{Introduction}
% \clearpage



% \section{Outputs and Normal Dynamics}

% \begin{comment}
%     I think it makes sense to be specific to robotic systems here instead of general control systems. Then we can constructively generate zero dynamics (which I think would be useful for roboticists to see) that are independent of the control input. Also, I think it just gets messy in the general case.

%     There exist conditions on the existence of outputs which render the system full-state feedback linearizeable, and therefore do not have zero dynamics \ref{sastry_linearization_1999}. These conditions are difficult to verify, but are in general not satisfied for many control systems of interest.

%     For underactuated systems, the rank deficiency of the matrix $\b B$ implies a lack of involutivity of the distribution $\b \Delta(\b x)$, and therefore an inability to choose any output $\b y$ which results in full state feedback linearizeability.
% \end{comment}

% Consider an $n-$degree of freedom robotic system with coordinates $\b q\in\mathcal{Q}$ and state $\b x = (\b q, \dot{\b q})\in \mathcal{X} \triangleq \mathsf{T}\mathcal{Q}.$ The dynamics can be written in control-affine form as:
% \begin{align}
%     \dot{\b x} = \underbrace{\begin{bmatrix} \dot {\b q} \\ \b D(\b q)^{-1} \b H(\b q, \dot{\b q}) \end{bmatrix}}_{\b f(\b x)} + \underbrace{\begin{bmatrix} \b 0 \\ \b D(\b q)^{-1} \b B\end{bmatrix}}_{\b g(\b x)}\b u \label{eq:robot_dynamics}
% \end{align}
% where $\b D : \mathcal{Q} \to \R^{n\times n}$ is the positive-definite mass-inertia matrix, $\b H:\mathcal{X} \to\R^n$ contains the Coriolis and gravity terms, $\b B\in\R^{n\times m}$ is the selection matrix, and $\b u\in\R^m$ is the control input. Many systems of interest -- e.g. legged robots, dexterous manipulators, and systems with strict actuator limits --  are \textit{underactuated}, meaning they have fewer actuators than degrees of freedom ($m < n$). Importantly, restricted actuation authority does not imply a loss of stabilizability; however, achieving stable behaviors requires careful coordination of the actuated degrees of freedom. For the following discussion we assume that $\b B$ has (column) rank $m$, and will be interested in stabilizing these underactuated systems to a goal position $\b x^*$.

% % (or more generally a control-invariant set $\Omega$),
% Towards this goal, it is convenient to construct a collection of outputs $\b y:\mathcal{X}\to \R^p$ via:
% \begin{align*}
%     \b y(\b x) = \b y_a(\b x) - \b y_d(\b x).
% \end{align*}
% In contrast to the typical perspective of outputs as observers \cite{kalman_new_1960}, we will instead be interested in outputs for which there exist constructive stabilization techniques. Synthesizing a control input to drive these outputs to zero requires $\b u$ to appear into a derivative of the output in a meaningful way. To make this precise, consider a time derivative of the output:
% \begin{align*}
%     \dot {\b y}(\b x) = \underbrace{\frac{\partial \b y}{\partial \b x}\b f(\b x)}_{L_\b f \b y(\b x)} + \underbrace{\frac{\partial \b y}{\partial \b x}\b g(\b x)}_{L_\b g \b y(\b x)} \b u 
% \end{align*}
% where $L_\b {f}\b y:\mathcal{X} \to \R^p$ and $L_\b {g}\b y:\mathcal{X} \to\R^{p\times m}$ are the \textit{Lie derivatives} of the output $\b y_a$ with respect to the vector fields $\b f$ and $\b g$, respectively. If the matrix $L_\b g \b y(x) $ is singular, we can attempt to continue differentiating until it is not:
% \begin{align*}
%     {\b y}^{(\gamma)}(\b x) &= L_\b f^\gamma(\b x) + L_\b gL_\b f^{\gamma-1}(\b x) \b u.
%     % \ddot{\b y} &= \underbrace{\b D(\b q)^{-1}\b H(\b q, \dot{\b q})}_{L_\b f^2 \b y_a(\b x)} + \underbrace{\b D(\b q)^{-1}\b B}_{L_\b g L_\b f \b y_a(\b x)}\b u.
% \end{align*}
% Differentiating the output until the input appears is captured in the following notion of strict relative degree:
% \begin{definition}
%     \cite{sastry_linearization_1999}
%     An output $\b y :\mathcal{X} \to \R^p$ for the system \eqref{eq:robot_dynamics} is said to have strict vector relative degree $\gamma\in\mathbb{N}$ at $\b x_0$ if:
%     \begin{align*}
%         L_{\b g_i}L_{\b f}^k \b y_i(\b x, t) \equiv 0,\ \ \ \ 0\le k\le \gamma-2
%     \end{align*}
%     for $i=1,\ldots p$ and the matrix $L_\b g L_\b f^{\gamma-1} \b y(\b x, t)$ is nonsingular for all $t\in\R_+$.
% \end{definition}

% The power of having a valid relative degree is that we can easily define a stabilizing controller, for example the following feedback linearizing controller:
% \begin{align}
%     \b u = L_\b g L_\b f^{\gamma-1} \b y(\b x)^{-1}(- L_\b f^\gamma \b y(\b x) + \b v), \label{eq:fbl}
% \end{align}
% whereby the auxiliary input $\b v$ can be chosen such that the resulting output dynamics ${\b y^{(\gamma)}} = \b v$ are exponentially stable. To make this more precies, defDefinineg the following output coordinates as:
% \begin{align*}
%     \b \eta(\b x) = \b\Phi_\eta(\b x)= \begin{bmatrix}
%         \b \eta^1 \\ \b\eta^2 \\ \vdots \\ \b\eta^{\gamma-1}
%     \end{bmatrix} \triangleq \begin{bmatrix}
%         \b y_a(\b x) \\ \dot{\b y}_a(\b x) \\ \vdots \\ {\b y}_a^{(\gamma-1)}(\b x)
%     \end{bmatrix}.
% \end{align*}
% where $\b y^{(j)}_a(\b x) = L_{\b f}^j\b y_a(\b x)$ for $j=1,\ldots,\gamma-1$ by the relative degree assumption. The output dynamics can be expressed as:
% \begin{align*}
% 	\dot{\b \eta} = \underbrace{\begin{bmatrix}\b 0 & \b I \\ \b 0 & \b 0\end{bmatrix}\b \eta + \begin{bmatrix} \b 0 \\ L_\b f^ \gamma\b y_a(\b x)\end{bmatrix}}_{\hat {\b f}(\b \eta,\b z)} + \underbrace{\begin{bmatrix} \b 0 \\ L_\b gL_\b f^{\gamma-1}\b y_a(\b x)\end{bmatrix}}_{\b{\hat g}(\b \eta, \b z)}\b u.
% \end{align*}
% Defining the error as $\b e \triangleq \b \eta - \b \eta_d$, The error dynamics under the feedback linearizing controller are given by:
% \begin{align}
% 	\dot{\b e} = \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 & \b 0 \end{bmatrix}}_{\triangleq \b F}\b e+ \underbrace{\begin{bmatrix}\b 0 \\ \b I\end{bmatrix}}_{\triangleq \b G}\b v
% \end{align}
% Given positive definite matrices $\b{Q} \in \R^{\gamma\times\gamma}$ and $\b R \in \R^{m\times m}$, we can solve the continuous algebraic Riccati equation (CARE):
% \begin{align*}
% 	\b F^\top \b P + \b P \b F - \b P \b B \b R^{-1} \b B^\top \b P = -\b Q
% \end{align*}
% for a positive definite symmetric matrix $\b P\in\R^{\gamma\times\gamma}$. This yields an auxiliary input defined by, we can for example take the auxiliary control to be $\b v = -\b R^{-1} \b B^\top \b P \b e$ and Lyapunov function $V = \b e^\top \b P \b e$ certifying the exponential stability of the output coordinates.




% % to exponentially stabilize $\b y_a(\b x)$ to $\b y_d(\b x, t)$. whereby and the.  -- make this point later
% % Related to this notion, we now introduce the idea of a desired output being dynamically feasbile:
% % \begin{definition}
% % 	A desired output $\b y_d:\mathcal{X}\to\R^p$ is \textit{dynamically feasible} if there exists a control input $\b u\in\R^m$ such that:
% % 	\begin{align*}
% % 		\dot {\b y}_d (\b x) = 
% % 	\end{align*}
% % \end{definition}K \b \eta$.
% % to exponentially stabilize $\b y_a(\b x)$ to $\b y_d(\b x, t)$. whereby and the.  -- make this point later

% With the goal of stabilizing to an equilibrium point $\b x^* = [\b q^*, \b 0]$, a natural choice of outputs would be $\b y_a(\b q) = \b q$ and $\b y_d \equiv \b q^*$, whereby we are directly requesting that the joint coordinates converge to a desired state. A quick computation shows that $L_\b {g}\b y_a(\b x) = \b 0$, and differentiating again, $L_\b {g}L_\b f\b y_a(\b x) = \b D(\b q)^{-1}\b B$. Because $\b B$ is rank deficient by virtue of the system being underactuated, this output does not have a valid relative degree. 
% % , making stabilization of arbitrary goal positions challenging. 
% For underactuated robotic systems, it is often challenging if not impossible to find output coordinates which span the complete state space and which can be feedback linearized \cite{bedrossian_nonlinear_nodate}. Even if such coordinates exist, verifying the algebraic conditions required to identify them is difficult \cite{isidori_elementary_1995-1}. In light of this, we will focus on producing coordinates which are of valid relative degree, and which when tracked will result in stability of the complete system.
% % A detailed discussion of this can be found in the Appendix. 

% Instead of viewing outputs as the primary objectives that we would like to converge to zero, we will use them as a proxy for characterizing the subspace of the system dynamics which the actuators directly effect. With this viewpoint in mind, consider the following outputs:
% \begin{align}
%     \b y_a(\b q) = \b B^\top \b q, \label{eqn:outputs}
% \end{align}
% whereby $L_\b g L_\b f^{\gamma-1} \b y_a(\b x) = \b B^\top \b D(\b q) \b B$ is an $m\times m$ block of the mass-intertia matrix and is therefore full rank at all points in the state space. Thus, these outputs have strict vector relative degree 2, and can be constructively stabilized via collocated feedback linearization.

% As we care about stabilizing $\b x$ and not just $\b y_a(\b x)$, however, we would like to know how stabilizing the outputs effects the complete system state. In order to make conclusions in the original state space, we need to reason about the following subspace:
% \begin{align*}
%     \mathcal{Z} = \{ \b x \in \R^n~|~ \b y_a(\b x) = \cdots = \b y_a^{(\gamma-1)}(\b x) = 0\}.
% \end{align*}
% Although producing a coordinate basis for $\mathcal{Z}$ can be challenging in general \cite{isidori_elementary_1995-1}, the structure of $\eqref{eq:robot_dynamics}$ and the outputs defined in \eqref{eqn:outputs} enable us to do this in a straightforward way. Choosing a matrix $\b N\in\R^{(n-m)\times m}$ to be a basis for the left nullspace of $\b B$, coordinates can be generated via:
% % which represent a codimension $p$ submanifold in $\R^n$ defining the set of states not directly affected by actuation. 
% % . There exist powerful result from geometric nonlinear control gives conditions on the existence of such coordinates, but these often result in verifying messy algebraic equalities. 
% % Conveniently, for robotic systems with the structure of $\eqref{eq:robot_dynamics}$ such coordinates can be constructively generated
% % by choosing the matrix $\b N\in\R^{(n-m)\times m}$ to be a basis for the left nullspace of $\b B$. With this, coordinates are given by:
% \begin{align*}
%     \b z(\b x) = \b\Phi_\b z(\b x) \triangleq\begin{bmatrix} \b N \b q \\ \b N \b D(\b q) \dot{\b q}\end{bmatrix}.
% \end{align*}
% These coordinates were chosen such that $\frac{d\b\Phi_\b z}{d \b x} \b g(\b x) \equiv \b 0$; as such, this mapping explicitly decomposes the state space into a subspace that can directly be controlled, and one that cannot. To transfer conclusions from the $(\b \eta, \b z)$ space to the original state space, we require that the map between them is bijective, as summarized in the following statement:
% \begin{proposition}
% \label{prop:bijection}
% The mapping $\b \Phi$ defined as:
% \begin{align*}
%     \begin{bmatrix} \b \eta(\b x) \\ \b z(\b x)\end{bmatrix} = \b \Phi(\b x) \triangleq \begin{bmatrix} \b \Phi_\eta(\b x) \\ \b\Phi_z(\b x)\end{bmatrix},
% \end{align*}
% is a diffeomorphism between $\mathcal{X}$ and $\mathcal{N}\times\mathcal{Z}$.
% \end{proposition}

% % Finally, applying the feedback linearizing controller from \eqref{eq:fbl}, 
% Finally, the associated dynamics in $(\b \eta, \b z)$ space are:
% \begin{align}
%     % \dot{\b \eta} &= \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 &\b 0 \end{bmatrix} \b \eta + \begin{bmatrix}\b 0 \\ L_{\b f}^\gamma\b y_a(\b \Phi^{-1}(\b \eta, \b z)) \end{bmatrix}}_{\hat{\b f}(\b \eta, \b z)} + \underbrace{\begin{bmatrix}\b 0 \\ L_\b gL_{\b f}^\gamma-1\b y_a(\b \Phi^{-1}(\b \eta, \b z))\end{bmatrix}}_{\hat{\b g}(\b \eta, \b z)}\b u, \\
%     % \dot{\b \eta} &= \underbrace{\begin{bmatrix} \b 0 & \b I \\ \b 0 &\b 0 \end{bmatrix}}_{\triangleq\b F} \b \eta + \underbrace{\begin{bmatrix} \b 0 \\ \b I \end{bmatrix}}_{\triangleq\b G} \b v, \ \ \ \ \ \ 
%     % \dot{\b z} = \underbrace{D\Phi_z \b f(\b \Phi^{-1}(\b \eta, \b z))}_{\triangleq\b \omega(\b \eta, \b z)}.
%     \dot{\b \eta} &= \hat{\b f}(\b \eta, \b z) +\hat{\b g}(\b \eta, \b z) \b u, \ \ \ \ \ \ 
%     \dot{\b z} = \underbrace{D\Phi_z \b f(\b \Phi^{-1}(\b \eta, \b z))}_{\triangleq\b \omega(\b \eta, \b z)}. \label{eqn:zd}
% \end{align}
% Conveniently, for the proposed choice of outputs and normal coordinates, constructing the function $\b\Phi^{-1}$ is straightforward.
% The next section will discuss the benefit of decomposing the system this way as a method of structuring stabilizing feedback policies.

% \section{Zero Dynamics Policies}
% \subsection{Optimal Control}

% The main objective of this work is to construct a feedback controller $\b u(\b x)$ which renders an equilibrium point $\b x^*$ exponentially stable for the underactuated system \eqref{eq:robot_dynamics}. As asymptotic stability is a necessary condition for optimality\footnote{Under the mild assumption that the system is observable under the state stage cost.}\cite{liberzon_calculus_2012}, one such controller is the solution to the infinite time optimal control problem, which can be written in $\b \eta$ and $\b z$ coordinates as:
% \begin{align}
%     % \b u^*(\b \eta, \b z)
%     V(\b\eta, \b z) \triangleq \min_{\substack{\b u(\cdot), \b \eta(\cdot), \b z(\cdot)}}\quad & \int_0^\infty h(\b \eta(\tau), \b z(\tau), \b u(\tau))d\tau \label{eqn:ftocp}\\
% \textrm{s.t.} \quad & \dot {\b \eta} = \hat {\b f}(\b \eta, \b z) + \hat{\b g}(\b \eta, \b z) \b u \notag\\
% & \dot{\b z} = \b\omega(\b \eta, \b z) \notag \\ 
%  \quad & (\b \eta(0), \b z(0)) = (\b \eta, \b z) \notag
% \end{align}
% By analyzing the above program, we are using the notion of optimality as a proxy for stability. Furthermore, we know that the time derivative of the optimal solution satisfies:
% \begin{align}
%     % \min_\b u \left(\dot V(\b \eta, \b z, \b u) + {h}(\b \eta, \b z, \b u) \right)= 0 \label{eqn:hjb}
% 	\min_\b u \Bigl(\underbrace{\begin{bmatrix}\frac{dV}{d\b\eta} \\ \frac{dV}{d\b z}\end{bmatrix}^\top\begin{bmatrix} \hat{\b f}(\b \eta, \b z) + \hat{\b g}(\b \eta, \b z)\b u \\ \b\omega(\b \eta, \b z)\end{bmatrix}}_{\dot V(\b \eta, \b z, \b u)} + {h}(\b \eta, \b z, \b u) \Bigr)= 0. \label{eqn:hjb}
% \end{align}
% Assuming that $h$ is positive definite with respect to all arguments, the resulting function $V$ will similarly be positive definite \red{cite}. Furthermore, for the minimizer $\b u^*$, we have that there exists a constant $c>0$ such that:
% \begin{align*}
% 	    \dot V(\b \eta, \b z, \b u^*) = - {h}(\b \eta, \b z, \b u^*) \le -c V(\b \eta, \b z), \label{eqn:zd_stab}
% \end{align*}
% and therefore serves as a Lyapunov function certifying the exponential stability of the overall system under the optimal control action. 

% There are two methods of solving the above optimal control problem: either getting pointwise estimates of $V$ by solving \eqref{eqn:ftocp} in a receding horizon fashion via MPC, or solving globally for a function $V$ satisfying \eqref{eqn:hjb} via the Hamilton-Jacobi-Bellman PDE. 
% % Both of these approaches suffer from dimensionality issues, as the total state space may be large for systems of interest. 
% To combat dimensionality and issues with online computational overhead, we will develop a method which exploits the aforementioned output and zeroing structure present in \eqref{eqn:zd}. Specifically, we propose finding a function $\func:\mathcal{Z}\to\mathcal{N}$ mapping between the underactuated and actuated coordinates, which draws inspiration from many successful results in robotics \red{raibert, centroidal MPC, backstepping, sliding mode control}. The zeroing manifold of such a function is defined as:
% \begin{align*}
%     \mathcal{M} \triangleq \{(\b \eta, \b z)\in \mathcal{N}\times\mathcal{Z}~|~ \underbrace{\b \eta - \func(\b z)}_{\triangleq h(\b \eta, \b z)}= \b 0\},
% \end{align*}
% which we require to be invariant under optimal control action. Assuming valid rank of $\b\psi$, $\mathcal{M}$ is an embedded submanifold of codimension equal to $\text{dim}(\mathcal{N})$. In order for this manifold to be invariant, we require that $\dot {\b x} \in \textsc{T} _\b x\mathcal{M}$, which can equivalently by written as $$\langle\partial \b e, \dot {\b x}\rangle|_{\b x\in\mathcal{M}} = 0$$ as the gradient field of a function provides a basis for the annihilator of its tangent space. In doing so, we will be able to use output tracking to this manifold to recover stability and bounded suboptimality of the overall system. 

% Suppose for the moment that such a function $\func$ exists with $\func(\b 0) = \b 0$ -- we will begin by analyzing the properties of this function, and will later provide constructive means of generating it. Invariance of $\mathcal{M}$ under optimal control implies:
% \begin{align*}
% 	    \hat{\b f}(\b \psi(\b z), \b z) + \hat{\b g}(\b \psi(\b z), \b z) \b u^*(\b z) = \frac{d\b\psi}{d\b z} \b\omega(\b \psi(\b z), \b z). \label{eqn:inv}
% \end{align*}
% where $\b u^*$ is the minimizer of \eqref{eqn:hjb} at the point $(\func(\b z), \b z)$.

% \begin{lemma}
%     Initial conditions on the manifold are exponentially stable.
% \end{lemma}
% \begin{proof}
%     Define the Lyapunov function candidate:
%     \begin{align*}
%         V_z(\b z) \triangleq V(\b \psi(\b z), \b z).
%     \end{align*}
% 	As $V$ is positive definite on its domain, is is stil positive definite when restricted to $\mathcal{M}$, and therefore $V_z$ is positive definite by construction. Taking the time derivative of $V_z$ yields:
% 	\begin{align*}
% 		\dot V_z = \frac{dV}{d\b\eta}\frac{d\b \psi}{d\b z}\b\omega(\b \psi(\b z), \b z)+\frac{dV}{d\b z}\b \omega(\b\psi(\b z), \b z).
% 	\end{align*}
% 	Invariance under optimal control in \eqref{eqn:inv} results in the substitution:
% 	\begin{align*}
% 		\dot V_z &= \frac{dV}{d\b\eta}\left(\hat{\b f}(\b \psi(\b z), \b z) + \hat{\b g}(\b \psi(\b z), \b z) \b u^*(\b z)\right)+\frac{dV}{d\b z}\b \omega(\b\psi(\b z), \b z) \\
% 		&\le -cV_z(\b z),
% 	\end{align*}
% 	where the last line follows from \eqref{eqn:zd_stab} and plugging in the definition of $V_z$.. 
% \end{proof}
% Next, we require that the manifold is dynamically feasible, i.e. is able to be tracked with zero error. One way to ensure this is to only produce a function $\func_1:\mathcal{Z}\to\mathcal{N}_1$ and differentiate it $\gamma$ times when producing a control input. As higher derivatives of functions, especially learned ones, can be noisy, we instead propose learning outputs $\func_i:\mathcal{Z}\to\mathcal{N}_i$ whereby $\func = [\func_1(\b z)~\func_2(\b z)]^\top$. When learning separate functions, we require a differential constraint to be satisfied between them -- it turns out that the invariance under optimal control input achieves this naturally. This is summarized in the following statement:
% \begin{lemma}
% 	Invariance of the manifold under optimal control implies that it is dynamically feasible.
% \end{lemma}
% \begin{proof}
% 	Expanding $\langle \partial h, \dot{\b x}^*\rangle = 0$ for the dynamics in \eqref{eqn:zd} implies $\dot \eta = \frac{d\func}{d\b z}\b{\dot z}$, which upon exapnding via \eqref{eqn:zd} yeilds:
% 	\begin{align*}
% 		\begin{bmatrix} \b \eta_2 \\ \tilde{\b f}(\b \eta, \b z) + \tilde{\b g}(\b \eta, \b z)\b u^* \end{bmatrix}\Bigg|_{(\b \eta, \b z)\in\mathcal{M}} = \begin{bmatrix}\frac{d\func_1}{d \b z}\b\omega(\func(\b z), \b z) \\ \frac{d\func_2}{d \b z}\b\omega(\func(\b z), \b z) \end{bmatrix}.
% 	\end{align*}
% 	Therefore, we can conclude that $\b \eta_2^d = \dot{\b \eta}_1^d$, and consequently that the outputs $\func$ are dynamically feasible.
% \end{proof}

% As we will never be exactly on the zero dynamics manifold, we next require \end{proof}



% % In order to stabilize the system dynamics, we need to decide what structure $\b y_d$ should have. 
% % Taking $\b y_a$ to be defined as in \eqref{eqn:outputs}, we propose the following form for the desired outputs:
% % \begin{align*}
% %     \b \eta_d(\b z) \triangleq \begin{bmatrix}
% %         \b y_d(\b z) \\ \dot{\b y}_d(\b z) 
% %     \end{bmatrix}
% % \end{align*}
% % \begin{align*}
% %     \b \eta_d \triangleq \begin{bmatrix}
% %         \b y_d(\b z) \\ \dot{\b y}_d(\b z) \\ \vdots \\ \dot{\b y}_d^{(\gamma-1)}(\b z)
% %     \end{bmatrix}
% % \end{align*}
% % With this, we can define the following error coordinates:
% % \begin{align*}
% %     \b e(\b x) = \b\Phi_e(\b x) \triangleq \b\eta - \b \eta_d(\b z),
% % \end{align*}
% % and associated \textit{error nullspace} manifold $\mathcal{M}$:
% % \begin{align*}
% %     \mathcal{M} = \{\b x\in\R^n~|~ \b e (\b x) = \b 0\},
% % \end{align*}


% \begin{example}
%     Linear system. Show the LQR subspace exists.
% \end{example}
% The aforementioned analysis assume that such a surface exists. We will now show that locally, we know that it does.
% \begin{theorem}
%     There exists a ball $B_\epsilon(\b 0) \subset\R^n$ such that this manifold exists. Furthermore, $T_0\mathcal{M}$ is exactly the LQR subspace.
% \end{theorem}

% \begin{theorem}
%     Output feedback to this policy results in composite stability for the overall system.
% \end{theorem}
% % Specifically, for the outputs defined in \eqref{eqn:outputs}, we have the following structure:
% % \begin{align*}
% %     \b\eta_d^1(\b z) &= \b\psi(\b z)\\
% %     \b\eta_d^2(\b z) &= \frac{d\b\psi}{d\b z}(\b z)\b\omega(\b \eta_d, \b z),
% % \end{align*}
% % which unfortunately results in an implicit solve for the second $\b \eta_d$ coordinate. Instead of training a  policy for only $\b \psi$ and deriving $\b \eta^2_d$ from it, we can jointly learn policies $\b\psi_1$ and $\b \psi_2$ and enforce a differential constraint between them. This is captured by requiring that the signals are \textit{dynamically feasible}.
% % In order for the output coordinates to be able to track this desired signal, it must be \textit{dynamically feasible}, there must exist an input $\b u$ such that the desired trajectory satisfies the output dynamics:
% % \begin{align*}
%     % \b F\b\eta_d + \b G \b v = \frac{d\b\eta_d}{d\b z}\b\omega(\b \eta_d, \b z).
%     % \hat{\b f}(\b\eta_d, \b z) + \hat{\b g}(\b \eta_d, \b z)\b u = \frac{d\b\eta_d}{d\b z}\b\omega(\b \eta_d, \b z),
% % \end{align*}
% % which more explicitly can be written as:
% % \begin{align*}
%     % \b F\b\eta_d + \b G \b v = \frac{d\b\eta_d}{d\b z}\b\omega(\b \eta_d, \b z).
%     % \begin{bmatrix} \b \eta^2_d\\ \overline{\b f}(\b\eta_d, \b z) + \overline{\b g}(\b \eta_d, \b z)\b u\end{bmatrix}= \begin{bmatrix} \frac{d\b\eta^1_d}{d\b z}\b\omega(\b \eta_d, \b z) \\ \frac{d\b\eta^2_d}{d\b \eta}(\hat{\b f}(\b\eta_d, \b z) + \hat{\b g}(\b \eta_d, \b z)\b u)+\frac{d\b\eta^2_d}{d\b z}\b\omega(\b \eta_d, \b z)\end{bmatrix}.
% % \end{align*}
% % The above constraint ensures that the surface defined by $\b \eta_d$ is able to be rendered forward invariant. We also require that the error nullspace dynamics, also known as the zero dynamics:
% % \begin{align*}
% %     \dot {\b z} = \b\omega(\b\eta_d, \b z),
% % \end{align*}
% % are stable in the sense of Lyapunov. Under these two conditions, we have the following:

% The next section will be devoted to describing how to construct a policy $\b \eta_d$ which enforces the above two conditions.

% We will use the solution of the optimal control problem as a proxy for the construction of a Lyapunov function which certifies the stability of the zero dynamics. This is done to avoid proposing a Lyapunov function candidate and learning a policy which certifies it, the complexities of which are discussed in the Appendix. 

% % A powerful result from geometric nonlinear control gives conditions on the existence of coordinates $\b z(\b x)$ such that the map:

% % is a diffeomorphism. 

% \begin{problem}
%     Given a candidate Lyapunov function on the zero dynamics coordinates $V_z$, find a desired output policy $\b \eta_d(\b z)$ such that $\dot V_z \le -\gamma V_z$.
% \end{problem}

% \red{Now we discuss the fact that proposing a Lyapunov function candidate would be nonsense (especially in the context of hybrid systems or systems with input bounds), so we jointly learn the policy and the value function. As opposed to PPO, we can directly compute the advantage by using MPC. And because of the zero dynamics, we get a dimensionality reduction.}


% \begin{align*}
%     \min_{\theta}\left[ \mathbb{E}_{\b z} \left\| \partial \b h_\theta (\b z) \dot{\b \varphi}_{\b\theta}(\b z)\right\|^2\right]
% \end{align*}


% \section{Stability}
% The goal of this work is to synthesize a control input $\b u = \b k(\b x, t)$ which is able to guarantee the stability of the overall system $\eqref{eqn:eom}$. We will be interested in asymptotic stability, which is defined as follows:
% \begin{definition}
% An \textit{asymptotically stable equilibrium point} is a point $x^*$ such that $f(x^*) = 0$ and $\forall \epsilon>0,~\exists \delta>0$ such that:
% \begin{subnumcases}{||x_0-x^*|| < \delta ~ \Rightarrow ~}
%     \|\phi_T(x_0)-x^*\|<\epsilon \quad \forall T \geq 0 \label{eqn:asy} \\
%     \lim_{T\to \infty} ||\phi_T(x_0) - x^*|| = 0 \label{eqn:lim}
% \end{subnumcases}
% % \begin{align}
 
% % \begin{cases}

% % \end{cases}
% % \end{align}
% \end{definition}

% \begin{lemma}
%     Let $V_{\b e}(\b \eta)$ and $V_{\b z}(\b z)$ be Lyapunov functions certifying the asymptotic stability of $\dot {\b e} = \b F \b e + \b G \b v$ and $\dot{\b z} = \b\omega(\b \eta_d, \b z)$, respectively. Then, there exists a $\sigma > 0$ such that the composite Lyapunov function $\b V(\b \eta, \b z) = \sigma V_{\b e}(\b \eta) + V_{\b z}(\b z)$ certifies asymptotic stability of the combined system.
% \end{lemma}
% \begin{proof}
% \begin{align*}
%      \dot {\b V}(\b \eta, \b z) &= \sigma \dot V_{\b e}(\b \eta) + \dot V_{\b z}(\b z) \\
%      & \le -\sigma \gamma V_{\b e}(\b \eta) + \frac{dV_{\b z}}{d \b z}\b\omega(\b e, \b z) \\
%      & \le -\sigma \gamma V_{\b e}(\b \eta) + \left\|\frac{dV_{\b z}}{d \b z}\right\|L_{\b\omega}Me^{-\lambda t}\|\b e(0)\|\\
% \end{align*}
    
% \end{proof}




% \section{Progress on problem formulation(13-11-23)}

% Consider the canonical optimal control problem equivalently reformulated using zero dynamics diffeomorphism $\b \Phi(\b x) \to (\b \eta, \b z )$:

% \begin{minipage}[t]{0.5\textwidth}
% \begin{align}
%     \min_{\b u(\cdot), x(\cdot)} \quad & \int_0^\infty h(\b x(\tau), \b u(\tau))d\tau \\
% \textrm{s.t.} \quad & \dot {\b x} = \b f(\b x) + \b g(\b x) \b u \\
%  \quad & \b x(0) = \b x_0
% \end{align}
% \end{minipage}
% \begin{minipage}[t]{0.5\textwidth}
% \begin{align}
%     \min_{\b \eta(\cdot), \b z(\cdot), \b v(\cdot)} \quad & \int_0^\infty \hat{h}(\b \eta(\tau), \b v(\tau))d\tau\\
% \textrm{s.t.} \quad & \dot {\b \eta} = \b F \b \eta  + \b G \b v \\ 
%               \quad & \dot {\b z} =  \b \omega( \b \eta, \b z ) \\
%               \quad & \b \eta(0) = \b \eta_0 \\
%               \quad & \b z(0) = \b z_0  
% \end{align}
% \end{minipage}

% \subsection{Assumptions enumeration}
% Here I will list a series of assumptions that will justify the rest of the derivation.
% Notice that some will need to be justified.
% \begin{enumerate}
%     \item $\text{dim}(\b \eta) >> \text{dim}(\b z)$. This is the key for dimensionality reduction and we need to explicitly walk readers through why this always happens and how it results in a significant dimensionality reduction for the systems we are concerned with.
%     \item Since $\b \eta $ is feedback linearizable, we can drive it anywhere we want exponentially quickly. We thus need to drive it towards achieving a desirable property in $\b z$. We will thus call $\b z$ the canonical control coordinates. (Formalizing this). 
% \end{enumerate}
% \red{as the control input required to keep the manifold invariant is unique, we simply need to solve a qp to decide which input to use. If we are on the surface, then this is the optimal input.}
% \subsection{Problem Description}
% From the canonical control coordinates assumption, we conclude an optimal controller for the desired task satisfies the following equality:

% \begin{align}
%     \b \eta^* = \b \eta_d = \b \psi (\b z)
% \end{align}
% In other words, the output coordinates follow some desired trajectory which is solely a function of $\b z$. Since $\b \eta^* $ is a solution to the optimal control problem, it must be dynamically feasible:

% \begin{align}
%     \dot{ \b \eta }_d = \frac{\partial \b \psi }{\partial \b z}^\top \b \omega ( \b \eta_d, \b z ) &=  \b F \b \eta_d + \b G \b v^* 
% \end{align}

% We thus need to find a $\b \psi$ that solves the following differential equation:

% \begin{align}
%     \frac{\partial \b \psi }{\partial \b z}^\top \b \omega ( \b \psi(\b z), \b z ) = \b F \b \psi(\b z)
% \end{align}

% We could therefore consider the following loss function:

% \begin{align}
%     \mathbb{E}_{x0}\left[ \alpha \lVert \b \varphi(\b x_0; \b \psi) \rVert_2^2 + \beta \lVert \frac{\partial \b \psi }{\partial \b z}^\top \b \omega ( \b \psi(\b z), \b z ) - F \b \psi(\b z) \rVert_2^2 \right]
% \end{align}

% Where the second term is a dynamic consistency term for the desired $y_d$. This assumes that $\b\varphi$ is implemented with a feedback linearizing controller on $\b \eta$.
% % \input{Sections/WalkingAsBarriers}

% \section{Learning from Pontryagin Maximum Principle Trajectories}

% Assume we have sampled densely around the origin to produce a set of PMP trajectories which have running estimate of the value function. We will now address how to estimate the true value function from these trajectories. We will begin by noting the following features of PMP trajectories:

% \begin{enumerate}
%     \item For PMP trajectory $i$ the running cost of the value function is positive: $V_i(\bm{x}) \geq 0$.
%     \item If PMP trajectories intersect at a point, the minimum of the value functions is the value function.
% \end{enumerate}

% These two assumptions inspire the following noise model for the Value function measurements from PMP trajectories:

% \begin{align}
%     \hat{V} \triangleq V_{PMP}(x) &= V(x) + \epsilon \\
%     \epsilon &\geq 0 \\
%     \epsilon &\sim \mathcal{D}(x) \\
% \end{align}

% Where $\epsilon$ is a positive random variable with unknown distribution dependent on $x$. We will now attempt to derive a Maximum a Posteriori (MAP) estimator for $V$ given samples $(x_i,  \hat{V}_i)$ where I am approximate $V$ with $NN$:
% \begin{align}
%     \theta^* &= \argmax_{\theta} \prod_{i=1}^N p( \hat{V}_i \mid x_i, \theta) \\
%     &=  \argmax_{\theta} \sum_{i=1}^N \log p( \hat{V} \mid x_i, \theta) \\
%     &=  \argmax_{\theta} \sum_{i=1}^N \log \mathbbm{1}\{\hat{V}_i - NN_\theta(x_i) \geq 0\} \lambda \exp\{-\lambda\left(\hat{V}_i - NN_\theta(x_i)\right)\} \\
%     &=  \argmax_{\theta} \sum_{i=1}^N \log \mathbbm{1}_{\{\hat{V}_i \geq NN_\theta(x_i)\}} + \log \lambda -\lambda\left(\hat{V}_i - NN_\theta(x_i)\right) \\
%     &=  \argmin_{\theta} \sum_{i=1}^N -\log \mathbbm{1}_{\{\hat{V}_i \geq NN_\theta(x_i)\}} - \log \lambda + \lambda\left(\hat{V}_i - NN_\theta(x_i)\right) \\
% \end{align}
% \section{Appendix}
% \begin{proof}[Proof of Proposition \eqref{prop:bijection}]
%     Consider $D\b\Phi$, given by:
%     \begin{equation} 
% D\Phi(q, \dot{q}, t) = \begin{bmatrix}
% B^\top & 0 \\ 0 & B^\top \\ N & 0 \\ \frac{\partial}{\partial q} ND(q)\dot{q} & ND(q) \end{bmatrix}
% \end{equation}
% This Jacobian is full rank at all points in the state space and in time (this can be seen by rearranging the rows to create and identity element in the top left), and noting that $ND(q) = \begin{bmatrix} D_{11}(q) & D_{12}(q)\end{bmatrix}$ where $D_{11}(q)$ is the upper right $n-m \times n-m$ square block of the inertia matrix and is thus invertible. 
% \end{proof}

% \bibliographystyle{ieeetr}
% \balance
% \bibliography{references}

% % % \section{Related Work}

% % \input{Sections/Conclusion.tex}

% % \clearpage
% % \section{Acknowledgements} 
% % The authors would like to thank Murtaza Hathiyari for his assistance with hardware implementation.

% % % Acknowledgments---Will not appear in anonymized version
% % % \acks{We thank a bunch of people.}

% % %
% % \bibliography{Zero Dynamics Policies}







% \end{document}

==> pmp_learning.tex <==

\section{Progress on problem formulation(13-11-23)}

Consider the canonical optimal control problem equivalently reformulated using zero dynamics diffeomorphism $\b \Phi(\b x) \to (\b \eta, \b z )$:

\begin{minipage}[t]{0.5\textwidth}
\begin{align}
    \min_{\b u(\cdot), x(\cdot)} \quad & \int_0^\infty h(\b x(\tau), \b u(\tau))d\tau \\
\textrm{s.t.} \quad & \dot {\b x} = \b f(\b x) + \b g(\b x) \b u \\
 \quad & \b x(0) = \b x_0
\end{align}
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
\begin{align}
    \min_{\b \eta(\cdot), \b z(\cdot), \b v(\cdot)} \quad & \int_0^\infty \hat{h}(\b \eta(\tau), \b v(\tau))d\tau\\
\textrm{s.t.} \quad & \dot {\b \eta} = \b F \b \eta  + \b G \b v \\ 
              \quad & \dot {\b z} =  \b \omega( \b \eta, \b z ) \\
              \quad & \b \eta(0) = \b \eta_0 \\
              \quad & \b z(0) = \b z_0  
\end{align}
\end{minipage}

\subsection{Assumptions enumeration}
Here I will list a series of assumptions that will justify the rest of the derivation.
Notice that some will need to be justified.
\begin{enumerate}
    \item $\text{dim}(\b \eta) >> \text{dim}(\b z)$. This is the key for dimensionality reduction and we need to explicitly walk readers through why this always happens and how it results in a significant dimensionality reduction for the systems we are concerned with.
    \item Since $\b \eta $ is feedback linearizable, we can drive it anywhere we want exponentially quickly. We thus need to drive it towards achieving a desirable property in $\b z$. We will thus call $\b z$ the canonical control coordinates. (Formalizing this). 
\end{enumerate}
\red{as the control input required to keep the manifold invariant is unique, we simply need to solve a qp to decide which input to use. If we are on the surface, then this is the optimal input.}
\subsection{Problem Description}
From the canonical control coordinates assumption, we conclude an optimal controller for the desired task satisfies the following equality:

\begin{align}
    \b \eta^* = \b \eta_d = \b \psi (\b z)
\end{align}
In other words, the output coordinates follow some desired trajectory which is solely a function of $\b z$. Since $\b \eta^* $ is a solution to the optimal control problem, it must be dynamically feasible:

\begin{align}
    \dot{ \b \eta }_d = \frac{\partial \b \psi }{\partial \b z}^\top \b \omega ( \b \eta_d, \b z ) &=  \b F \b \eta_d + \b G \b v^* 
\end{align}

We thus need to find a $\b \psi$ that solves the following differential equation:

\begin{align}
    \frac{\partial \b \psi }{\partial \b z}^\top \b \omega ( \b \psi(\b z), \b z ) = \b F \b \psi(\b z)
\end{align}

We could therefore consider the following loss function:

\begin{align}
    \mathbb{E}_{x0}\left[ \alpha \lVert \b \varphi(\b x_0; \b \psi) \rVert_2^2 + \beta \lVert \frac{\partial \b \psi }{\partial \b z}^\top \b \omega ( \b \psi(\b z), \b z ) - F \b \psi(\b z) \rVert_2^2 \right]
\end{align}

Where the second term is a dynamic consistency term for the desired $y_d$. This assumes that $\b\varphi$ is implemented with a feedback linearizing controller on $\b \eta$.
% \input{Sections/WalkingAsBarriers}

\section{Learning from Pontryagin Maximum Principle Trajectories}

Assume we have sampled densely around the origin to produce a set of PMP trajectories which have running estimate of the value function. We will now address how to estimate the true value function from these trajectories. We will begin by noting the following features of PMP trajectories:

\begin{enumerate}
    \item For PMP trajectory $i$ the running cost of the value function is positive: $V_i(\bm{x}) \geq 0$.
    \item If PMP trajectories intersect at a point, the minimum of the value functions is the value function.
\end{enumerate}

These two assumptions inspire the following noise model for the Value function measurements from PMP trajectories:

\begin{align}
    \hat{V} \triangleq V_{PMP}(x) &= V(x) + \epsilon \\
    \epsilon &\geq 0 \\
    \epsilon &\sim \mathcal{D}(x) \\
\end{align}

Where $\epsilon$ is a positive random variable with unknown distribution dependent on $x$. We will now attempt to derive a Maximum a Posteriori (MAP) estimator for $V$ given samples $(x_i,  \hat{V}_i)$ where I am approximate $V$ with $NN$:
\begin{align}
    \theta^* &= \argmax_{\theta} \prod_{i=1}^N p( \hat{V}_i \mid x_i, \theta) \\
    &=  \argmax_{\theta} \sum_{i=1}^N \log p( \hat{V} \mid x_i, \theta) \\
    &=  \argmax_{\theta} \sum_{i=1}^N \log \mathbbm{1}\{\hat{V}_i - NN_\theta(x_i) \geq 0\} \lambda \exp\{-\lambda\left(\hat{V}_i - NN_\theta(x_i)\right)\} \\
    &=  \argmax_{\theta} \sum_{i=1}^N \log \mathbbm{1}_{\{\hat{V}_i \geq NN_\theta(x_i)\}} + \log \lambda -\lambda\left(\hat{V}_i - NN_\theta(x_i)\right) \\
    &=  \argmin_{\theta} \sum_{i=1}^N -\log \mathbbm{1}_{\{\hat{V}_i \geq NN_\theta(x_i)\}} - \log \lambda + \lambda\left(\hat{V}_i - NN_\theta(x_i)\right) \\
\end{align}
